AutoPrep: Natural Language Question-Aware Data Preparation with a Multi-Agent Framework

Answering natural language (NL) questions about tables, known as Tabular Question Answering (TQA), is crucial because it allows users to quickly and efficiently extract meaningful insights from structured data, effectively bridging the gap between human language and machine-readable formats. Many of these tables are derived from web sources or real-world scenarios, which require meticulous data preparation (or data prep) to ensure accurate responses. However, preparing such tables for NL questions introduces new requirements that extend beyond traditional data preparation. This question-ware data preparation involves specific tasks such as column derivation and filtering tailored to particular questions, as well as question-aware value normalization or conversion, highlighting the need for a more nuanced approach in this context. Because each of the above tasks is unique, a single model (or agent) may not perform effectively across all scenarios. In this paper, we propose AutoPrep, a large language model (LLM)-based multiagent framework that leverages the strengths of multiple agents, each specialized in a certain type of data prep, ensuring more accurate and contextually relevant responses. Given an NL question over a table, AutoPrep performs data prep through three key components. Planner: Determines a logical plan, outlining a sequence of high-level operations. Programmer: Translates this logical plan into a physical plan by generating the corresponding low-level code. Executor: Executes the generated code to process the table. To support this multi-agent framework, we design a novel Chain-ofClauses reasoning mechanism for high-level operation suggestion, and a tool-augmented method for low-level code generation.

==> figures/tex/case_study.tex <==
\begin{figure*}[t]
    % \vspace{-1em}
    \centering
    \begin{subfigure}{0.48\textwidth}
        \includegraphics[width=\textwidth]{figures/fig/app-case_study1.pdf}
        % \captionsetup{skip=0.5pt}
        \caption{Case one}
        \label{fig:case_study1}
    \end{subfigure}
    \hspace{-1mm}
    \quad \quad
    \begin{subfigure}{0.48\textwidth}
        \includegraphics[width=\textwidth]{figures/fig/app-case_study2.pdf}
        % \captionsetup{skip=0.5pt}
        \caption{Case two}
        \label{fig:case_study2}
    \end{subfigure}
    \vspace{-2.5em}
    \caption{{Two case studies selected from TabBench and WikiTQ to qualitatively analyze effectiveness of \sys.}}
    \label{fig:case_study}
    \vspace{-1em}
\end{figure*}

==> figures/tex/executor_debugger.tex <==
%!TEX root = ../../main.tex
\begin{figure}[!t]
    \centering 
    \includegraphics[width=0.9\columnwidth]{figures/fig/executor_debugger.pdf}
    % \vspace{-1em}
    \caption{The executing and debugging process of operators. It contains two steps, (1) Pre-Diagnosis and (2) Executing the operators on relative tables.}
    \label{fig:executor_debugger}
    \vspace{-1em}
\end{figure}

==> figures/tex/pseudo_code_analysis_based_planner.tex <==
%!TEX root = ../../main.tex
\begin{figure}[!t]
    \centering 
    \includegraphics[width=0.99\columnwidth]{figures/fig/pseudo_code_analysis_based_planner.pdf}
    \vspace{-1em}
    \caption{Pseudo Code Analysis based Planner.}
    \label{fig:pseudo_code_analysis_based_planner}
    \vspace{-1em}
\end{figure}

==> figures/tex/pseudo_code_instance.tex <==
%!TEX root = ../../main.tex
\begin{figure}[!t]
    \centering 
    \includegraphics[width=0.99\columnwidth]{figures/fig/pseudo_code_instance.pdf}
    \vspace{-1em}
    \caption{Generated pseudo code.}
    \label{fig:pseudo_code_instance}
    \vspace{-1em}
\end{figure}

==> figures/tex/table_wrangling_agent.tex <==
%!TEX root = ../../main.tex
\begin{figure*}[!t]
    \centering 
    \includegraphics[width=0.99\textwidth]{figures/fig/table_wrangling_agent.pdf}
    % \vspace{-1em}
    \caption{An instance of illustrating the implementation of agents in table wrangling. \textbf{Profile (a)} illustrate the design of Planner. \textbf{Profile (b)} and \textbf{Profile (c)} define the working pipeline of Derive and Normalize. After receiving the requirements, these agents generate operators with arguments which will be fed to the Executor to process the table.}
    \label{fig:agent_implementation}
    \vspace{-1em}
\end{figure*}

==> plots/tex/_in_response_subcategories_in_other.tex <==
%!TEX root = ../../main.tex
\begin{figure}[!t]
    \centering 
    \includegraphics[width=0.99\columnwidth]{plots/plot/subcategories_in_other.pdf}
    \vspace{-1em}
    \caption{{In-depth Analysis of the ``\term{Other}'' Category.}
    }
    \label{fig:_in_response_subcategories_in_other}
    \vspace{-1em}
\end{figure}


==> plots/tex/_in_response_time_money_acc_scatter_map.tex <==
% \begin{figure}[!t]
%     % \vspace{-1em}
%     \centering
%     \begin{subfigure}{0.49\columnwidth}
%         \includegraphics[width=\textwidth]{plots/plot/time_money_acc_scatter_map_small_table.pdf}
%         % \captionsetup{skip=-0.3pt}
%         % \caption{Small Tables}
%         \label{fig:time_money_acc_scatter_map_small_table}
%     \end{subfigure}
%     \hspace{0.2mm}
%     % \quad
%     \begin{subfigure}{0.49\columnwidth}
%         \includegraphics[width=\textwidth]{plots/plot/time_money_acc_scatter_map_large_table.pdf}
%         % \captionsetup{skip=-0.3pt}
%         % \caption{Large Tables}
%         \label{fig:time_money_acc_scatter_map_large_table}
%     \end{subfigure}
%     \vspace{-4em}
%     \caption{\revise{Efficiency evaluation. The X-axis and y-axis represent the time cost (s) and monetary cost (\$) for processing one instance. The color intensity of scatters indicates the overall accuracy.}}
%     \label{fig:time_money_acc_scatter_map}
%     % \vspace{-1.5em}
% \end{figure}

%!TEX root = ../../main.tex
\begin{figure}[!t]
    \centering 
    \includegraphics[width=0.99\columnwidth]{plots/plot/time_money_acc_scatter_map.pdf}
    \vspace{-1em}
    \caption{{Efficiency evaluation. 
    The $x$-axis and $y$-axis represent the time cost (in seconds) and monetary cost (in dollars) for processing a single instance, respectively. The color intensity of each scatter point reflects the overall accuracy, with darker colors indicating higher accuracy.}
 %   The $x$-axis and $y$-axis represent the time cost (s) and monetary cost (\$) for processing one instance. The color intensity of scatters indicates the overall accuracy.}
    }
    \label{fig:_in_response_time_money_acc_scatter_map}
    \vspace{-1em}
\end{figure}


==> plots/tex/acc_on_table_with_different_complex_question.tex <==
\begin{figure}[!t]
    % \vspace{-1em}
    \centering
    \begin{subfigure}{0.49\columnwidth}
        \includegraphics[width=\textwidth]{plots/plot/accuracy_on_simple_tabfact.pdf}
        \captionsetup{skip=-0.5pt}
        \caption{Simple Question}
        \label{fig:accuracy_on_simple_tabfact}
    \end{subfigure}
    \hspace{0.2mm}
    % \quad
    \begin{subfigure}{0.49\columnwidth}
        \includegraphics[width=\textwidth]{plots/plot/accuracy_on_complex_tabfact.pdf}
        \captionsetup{skip=-0.5pt}
        \caption{Complex Question}
        \label{fig:accuracy_on_complex_tabfact}
    \end{subfigure}
    \vspace{-2em}
    \caption{{Comparison of \sys and other data prep methods on  questions with different difficulties in TabFact.}}
    \label{fig:acc_on_table_with_different_complex_question}
    \vspace{-1em}
\end{figure}


==> plots/tex/acc_on_table_with_different_size.tex <==
% %!TEX root = ../../main.tex
% % \begin{figure}[!t]
% %     \centering 
% %     \includegraphics[width=0.99\columnwidth]{plots/plot/comparison_of_methods_on_table_size.pdf}
% %     \vspace{-1em}
% %     \caption{}
% %     \label{fig:comparison_of_methods_on_table_size}
% %     \vspace{-1em}
% % \end{figure}

% \begin{figure}[!t]
%     % \vspace{-1em}
%     \centering
%     \begin{subfigure}{0.32\columnwidth}
%         \includegraphics[width=\textwidth]{plots/plot/accuracy_on_small_tables.pdf}
%         \captionsetup{skip=-0.3pt}
%         \caption{Small}
%         \label{fig:accuracy_on_small_tables}
%     \end{subfigure}
%     \hspace{0.2mm}
%     % \quad
%     \begin{subfigure}{0.32\columnwidth}
%         \includegraphics[width=\textwidth]{plots/plot/accuracy_on_medium_tables.pdf}
%         \captionsetup{skip=-0.3pt}
%         \caption{Medium}
%         \label{fig:accuracy_on_medium_tables}
%     \end{subfigure}
%     \hspace{0.2mm}
%     % \quad
%     \begin{subfigure}{0.32\columnwidth}
%         \includegraphics[width=\textwidth]{plots/plot/accuracy_on_large_tables.pdf}
%         \captionsetup{skip=-0.3pt}
%         \caption{Large}
%         \label{fig:accuracy_on_large_tables}
%     \end{subfigure}
%     \vspace{-2em}
%     \caption{\revise{Comparison of \sys and other data prep methods on tables with different sizes on the WikiTQ dataset.}}
%     \label{fig:comparison_of_methods_on_table_size}
%     \vspace{-1em}
% \end{figure}


%!TEX root = ../../main.tex
\begin{figure}[!t]
    \centering 
    \includegraphics[width=0.99\columnwidth]{plots/plot/accuracy_on_different_size_tables.pdf}
    \vspace{-1em}
    \caption{{Accuracy on different size of tables in WikiTQ.}
    %, such as NL2SQL as shown in the figure. \sys decomposes the data prep process into three stages: \textcircled{1} The Planning stage, \textcircled{2} the Programming stage and \textcircled{3} the Executing stage.
    }
    \label{fig:accuracy_on_different_size_tables}
    % \vspace{-1em}
\end{figure}

==> plots/tex/accuracy_on_meaningless_columns.tex <==


%!TEX root = ../../main.tex
\begin{figure}[!t]
    \centering 
    \includegraphics[width=0.7\columnwidth]{plots/plot/accuracy_on_meaningless_columns.pdf}
    \vspace{-1em}
    \caption{{Evaluation on dataset with meaningless columns.}
    %, such as NL2SQL as shown in the figure. \sys decomposes the data prep process into three stages: \textcircled{1} The Planning stage, \textcircled{2} the Programming stage and \textcircled{3} the Executing stage.
    }
    \label{fig:accuracy_on_meaningless_columns}
    \vspace{-1em}
\end{figure}


==> plots/tex/prompt_instance_generating_logical_requirement.tex <==
%!TEX root = ../../main.tex
\begin{figure}[!t]
    \centering 
    \includegraphics[width=0.99\columnwidth]{figures/fig/prompt_instance_generating_logical_requirement.pdf}
    \vspace{-0.5em}
    \caption{Details of Converting the Analyzer Sketch into Actions.}
    \label{fig:prompt_instance_generating_logical_requirement}
    \vspace{-1em}
\end{figure}

==> plots/tex/subcategories_in_other.tex <==


%!TEX root = ../../main.tex
\begin{figure}[!t]
    \centering 
    \includegraphics[width=0.99\columnwidth]{plots/plot/subcategories_in_other.pdf}
    \vspace{-1em}
    \caption{{In-depth Analysis of the ``\term{Other}'' Category.}
    %, such as NL2SQL as shown in the figure. \sys decomposes the data prep process into three stages: \textcircled{1} The Planning stage, \textcircled{2} the Programming stage and \textcircled{3} the Executing stage.
    }
    \label{fig:subcategories_in_other}
    % \vspace{-1em}
\end{figure}


==> plots/tex/tabbench_acc.tex <==
%!TEX root = ../../main.tex
\begin{figure}[!t]
    \centering 
    \includegraphics[width=0.9\columnwidth]{plots/plot/overall_accuracy_on_tabbench.pdf}
    \vspace{-1.5em}
    \caption{On TabBench.}
    \label{fig:overall_accuracy_on_tabbench}
    \vspace{-1em}
\end{figure}

==> response/_root.tex <==
%!TEX root = ../main.tex

\twocolumn

\clearpage
\pagenumbering{roman}


\renewcommand{\thetable}{\Roman{table}}
\renewcommand{\thefigure}{\Roman{figure}}
\setcounter{figure}{0}
\setcounter{table}{0}
% \clearpage
% \newpage

\input{response/general}
\input{response/r1}
\input{response/r2}
\input{response/r3}
\input{response/meta}


\renewcommand{\thetable}{\arabic{table}}
\renewcommand{\thefigure}{\arabic{figure}}
\setcounter{figure}{0}
\setcounter{table}{0}


\clearpage
\setcounter{page}{1}
\pagenumbering{arabic}




==> response/general.tex <==
%!TEX root = ../main.tex
\subsection*{Dear VLDB Meta-Reviewer and Reviewers,}

\noindent 
%We would like to thank the meta-reviewer and reviewers for the thorough reading of our paper and for your valuable comments.
%The paper has been revised according to the reviewers' comments, from clarifications to new datasets, new baseline and new experiments.
We sincerely thank the meta-reviewer and reviewers for their thorough reading and insightful feedback. 
In response, we have made substantial revisions to the paper, including clarifications, the introduction of new datasets, additional baselines, and new experiments.
The updated contents in the paper are highlighted in \revise{blue}.
Figures and tables in the response letter are numbered with Roman numerals (\eg Table I and Figure II), while those in the main paper use Arabic numerals (\eg Table 1 and Figure 2).

%The figures and tables in the response letter are numbered with Roman letters (\eg Table I, Figure II), while in the main paper are numbered with Arabic letters (\eg Table 1, Figure 2).

%Below, we first summarize the \textbf{main changes}, followed by \textbf{detailed responses} to the meta-reviewer and all reviewers.

Below, we first summarize the \textbf{main changes}, and then present \textbf{detailed responses} to each reviewer and the meta-reviewer.

\subsection*{Our Main Changes}

\stitle{M\modificationnum\label{modify:motivation} [Clarification on Motivation]:} 
We have revised the \textbf{Introduction} to more clearly justify our motivation.
Specifically, we clarified the data prep challenges in TQA.
To this end, we have updated \textbf{Figure~\ref{fig:error_instance_record}} by renaming the original categories \emph{column-level}, \emph{cell-level}, and \emph{table-level} to more precise terms: \emph{missing semantics}, \emph{inconsistent values}, and \emph{irrelevant columns}, respectively.
We have also revised the examples in \textbf{Figure~\ref{fig:issue_instances}} to better demonstrate typical data preparation issues and further clarify the connections between these issues and corresponding question-aware data prep tasks.

\stitle{M\modificationnum\label{modify:problem-novelty} [Justification on Problem Novelty]:}
We have revised the \textbf{Introduction} to better justify the novelty of \emph{question-aware data preparation}. Specifically, we highlight that, in contrast to traditional data preparation, question-aware data prep introduces a novel challenge, namely \emph{semantic alignment between structured tables and natural language questions}.


\stitle{M\modificationnum\label{modify:new-exps} [Seven Groups of New Experiments]:}
We have significantly revised the experimental sections in response to reviewer feedback, incorporating \textbf{seven new groups of experiments}.
%%
\begin{itemize}[leftmargin=15pt]
	\item[(1)] We have compared \sys with a new baseline, \textbf{Off-Prep}, which performs \emph{offline} data preparation on all tables in the TQA task. The experimental results are presented in \textbf{Table~\ref{tbl:vs_other_prep_method}}, with detailed analysis provided in \textbf{Exp-\ref{exp:compare_dataprep_baseline} of Section~\ref{subsec:Data_Prep_Method_Comparision}}.
	%
	\item[(2)] We have compared \sys with a new baseline \textbf{AutoTQA}~\cite{DBLP:journals/pvldb/ZhuCXLSZSTL24}, a SOTA TQA method that also adopts a multi-agent, LLM-based framework.
	The experimental results are reported in \textbf{Table~\ref{tbl:vs_other_prep_method}}, and detailed analysis is provided in \textbf{Exp-\ref{exp:compare_SOTA_TQA_with_prep} of Section~\ref{subsec:Data_Prep_Method_Comparision}}.
	%
	\item[(3)] We have evaluated the overhead of \sys in terms of both processing time and API cost, and compared it against baseline methods.
    The experimental results are reported in \textbf{Figure~\ref{fig:time_money_acc_scatter_map}}, with detailed analysis provided in \textbf{Exp-\ref{exp:efficiency_evaluation} of Section~\ref{subsec:efficiency_evaluation}}.
	%
	\item[(4)] We have evaluated the \emph{extensibility} of \sys for new operation types. The experimental results are reported in 
	\textbf{Table~\ref{tbl:new_operator_new_operation}} and detailed analysis is provided in \textbf{Exp-\ref{exp:scalability_exp_new_op_type} of Section~\ref{subsec:evaluation_on_generalization}}.	
	%
	\item[(5)] We have conducted new experiments to validate the superiority of our proposed framework \sys across different table sizes and various question difficulties. Due to space constraints, the detailed results and analysis are presented in \textbf{Appendix B.1 and B.2 of our technical report~\cite{technical_report}}.
	%
	\item[(6)] As discussed in Section~\ref{subsec:prog-idea}, we prompt the LLM to write code to implement the logical operation if no suitable function in the function pool can meet the requirement, which we denote as $\mathtt{CustomCode}$.
	To evaluate the effectiveness of LLM-based $\mathtt{CustomCode}$ in helping \sys generalize to cases that require new physical operations, we have conducted new experiments. Due to space constraints, the detailed experimental results and analysis are provided in \textbf{Appendix B.3 of our technical report~\cite{technical_report}}.
    \item[(7)] We have investigated the impact of additional data prep issues, \ie missing values and duplications, in TQA tasks. Due to space limitations, the corresponding experimental results are presented in \textbf{Appendix B.4 of our technical report~\cite{technical_report}}.
\end{itemize} 

\stitle{M\modificationnum\label{modify:error-analysis} [Details of Error Analysis]:}
We have provided detailed error analysis in Figure~\ref{fig:error_instance_record}, which serves as a key motivation for our proposed solution. Due to space limitations, the full analysis is presented in \textbf{Appendix A of our technical report~\cite{technical_report}}.

\stitle{M\modificationnum\label{modify:technical-details} [Technical Details]:}
We have revised \textbf{Sections~\ref{sec:the_planner_agent} and \ref{sec:the_programmer_and_executor}} to provide more comprehensive technical details. In addition, we have included all the detailed \textbf{LLM prompts}, which are presented in \textbf{Appendix D of our technical report~\cite{technical_report}} due to space limitations.

\stitle{M\modificationnum\label{modify:future-work} [Future Work]:}
We have revised \textbf{Section~\ref{sec:conclusion_and_future_work}} to identify three promising directions as our future work, \ie extending data prep capabilities of \sys,  supporting multi-table TQA, and enabling question-aware data preparation over enterprise datasets.

==> response/meta.tex <==
%!TEX root = ../main.tex
\subsection*{Responses to Meta-Reviewer}

We sincerely thank the Meta-Reviewer for the appreciation of our work.  
As suggested, we have carefully addressed all detailed comments and revision requests, and have made substantial improvements throughout the paper.

% \vspace{-1em}
\begin{shaded}
{
\stitle{MC1:} 
% Comprehensive discussion on extensibility and support for new operations types.
\emph{Comprehensive discussion on extensibility and support for new operations types.}
}
\end{shaded}

\noindent{\bf RESPONSE}:
% See the responses to \textbf{R2W1} \& \textbf{R3W1}.
We have added a \textbf{new experiment} to evaluate \sys on the extensibility of supporting new operation types and compare with other baseline methods. Please refer to the responses to \textbf{R2W1} \& \textbf{R3W1}.


\begin{shaded}
{
\stitle{MC2:} 
% Comparison with AutoTQA
\emph{Comparison with AutoTQA.}
}
\end{shaded}

\noindent{\bf RESPONSE}: 
% See the responses to \textbf{R1D13} \& \textbf{R2W3}.
We have added AutoTQA as a \textbf{new baseline} and conducted a thorough comparison with AutoTQA. Please see the responses to \textbf{R1D13} \& \textbf{R2W3}.



\begin{shaded}
{
\stitle{MC3:} 
% Comparison with offline cleaning approaches
\emph{Comparison with offline cleaning approaches.}
}
\end{shaded}

\noindent{\bf RESPONSE}: We have added a \textbf{new baseline} Off-Prep and thoroughly compare it with \sys. Please see the response to \textbf{R1R3}.


\begin{shaded}
{
\stitle{MC4:} 
% Better explain various technical details such as prompts
\emph{Better explain various technical details such as prompts.}
}
\end{shaded}

\noindent{\bf RESPONSE}: We have included \textbf{all detailed prompts}, which are presented in Appendix D of our technical report~\cite{technical_report} due to space limitations. Please see the responses to \textbf{R2W2} \& \textbf{R3W2}. We have also revised our paper to further clarify technical details that reviewers are concerned about. Please see the response to \textbf{R1D10}.


\begin{shaded}
{ 
\stitle{MC5:} 
% Experiments with overheads of a multi-agent approach such as processing time for complex data preparation operations
\emph{Experiments with overheads of a multi-agent approach such as processing time for complex data preparation operations.}
}
\end{shaded}

\noindent{\bf RESPONSE}: We have conducted a \textbf{new experiment} to evaluate the overhead of \sys in terms of both processing time and API cost, and compared it against baseline methods on tables with various sizes. Please refer to the response to \textbf{R3W3}.



==> response/r1.tex <==
%!TEX root = ../main.tex
\subsection*{Responses to Reviewer \#1}
\label{cover_letter:r1}

% 该reviewer不太认可question-aware data prep，认为offline data prep已足够
% 先要说明 question-aware data prep优于offline，这一点要立住脚，然后可以解决O15等问题

% \vspace{-1em}
\begin{shaded}
{
\stitle{R1R1:} \emph{Sufficiently explain the analysis presented in Fig. 1, including the "other" error category.}

\stitle{R1W1:} \emph{Error analysis (Fig. 1) not explained sufficiently, even though it forms the premise and motivation for the proposed system}

\stitle{R1D1:}
\emph{(1) The error analysis in Fig. 1 is not sufficiently explained. You use this as motivation for your solution, therefore it is very important for your argument. How was the analysis conducted? How were the error types extracted? What about the ``other'' category contributing 16\% or 24\% of errors? (2) The statement ``The above three types of operations address most of the errors caused by insufficient data prep, as shown in our error analysis in Figure 1.'' in particular remains unclear, as the connection is not recognizable. (3) What about missing values (cell-level) or duplicates (table-level), for example?}

}
\end{shaded}

\noindent{\bf RESPONSE}: 
We thank the reviewer for pinpointing this important issue. 
As suggested, we have provided a detailed explanation of the error analysis in Figure~\ref{fig:error_instance_record} (Our main change \textbf{M\ref{modify:error-analysis}}).

\stitle{Details of the Error Analysis.}
To better address the reviewer’s questions, we provide the following clarifications: (1) how the TQA process is conducted, (2) how the errors are categorized, and (3) what constitutes the “\term{Other}” category.

\etitle{(1) TQA Method: NL2SQL Based on GPT-4.}
We adopt NL2SQL~\cite{rajkumar2022evaluating}, a representative TQA baseline that does not perform data prep, as introduced in Section~\ref{subsec:exp-setup}. Specifically, given a natural language question $Q$ and a table $T$, we prompt GPT-4 to generate an SQL query $\term{SQL}$ using a few-shot in-context learning strategy. The query is then executed on $T$ to obtain the final answer $Ans$ for $Q$.

\etitle{(2) Error Categorization.}
We recruite three graduate students from our university's database group to annotate error categories for a randomly sampled set of 500 instances from WikiTQ and TabFact. All annotators have a good understanding of the TQA task and are proficient in SQL syntax.
We instruct the annotators to first identify errors stemming from insufficient data prep, assigning any remaining errors to a default category labeled \term{Other}. For the data prep-related errors, after careful investigation, we further categorize them into the following three types:
(1) \textbf{Missing Semantics:} The table lacks necessary semantic information required to accurately answer the NL question. 
(2) \textbf{Inconsistent Values:} Values within a column are represented inconsistently across different records. 
(3) \textbf{Irrelevant Columns:} The table includes many columns, but only a small subset are actually relevant to the NL question. 

\input{plots/tex/_in_response_subcategories_in_other}

\etitle{(3) In-depth Analysis of the ``\term{Other}'' Category}. 
We report the detailed sub-categories within the ``\term{Other}'' category in Figure~\ref{fig:_in_response_subcategories_in_other}. As shown, for WikiTQ, more than half of the cases stem from issues inherent to the dataset itself. Notably, 40\% of the errors are due to limitations in the evaluation function, where semantically equivalent but non-identical responses are marked as incorrect, a problem also highlighted in~\cite{cheng2023binding}. Additionally, 20\% of the errors arise from formatting issues in the model’s responses, where the generated SQL logic is correct but the output includes extraneous values from irrelevant columns.
On the other hand, for the TabFact dataset, most errors are attributed to model reasoning failures. Over 50\% result from the model’s inability to generate logically complete and accurate SQL queries. Furthermore, more than 35\% of the errors are due to response formatting issues, where the model returns ambiguous values instead of definitive true/false answers. 



%We have added details of the Error Analysis in \textbf{Appendix~\ref{sec:appendix_details_of_error_analysis}}. Specifically, we introduce the used TQA method, error extraction and labeling process. We also give a more detailed description about the ``Other'' category and provide specific cases for each sub-categories. In addition, we have conducted \textbf{a new experiment} to analyze the influence of duplicates and missing values.
%
%\stitle{Details of the error analysis.} We conduct the error analysis by implementing a wide adopted NL2SQL method based on GPT-4 for TQA task~\cite{rajkumar2022evaluating}. Then we hire 3 graduate students who are familiar with the TQA task and SQL syntax from the database group in our university to conduct error category labeling. Based on the granularities at which the data prep operation is required to conduct, i.e., the cell, the column, or the entire table, we categorize the errors into Cell-Level, Column-Level and Table-Level. Moreover, the ``other" category, as illustrated in Figure~\ref{fig:error_instance_record}, refers to error cases caused by factors unrelated to data prep. For example, the evaluation error in Table~\ref{tbl:wikitq_evaluation_error} is categorized into ``other'' where the evaluation function fails to match the correct prediction ``at Dallas Cowboys'' to the label ``Dallas Cowboys''. Considering that these errors are not the focus of this paper, we did not describe this in the Introduction for the readability of the draft.

\stitle{Connection Between the Errors and Logical Operations.}
We have revised \textbf{Section~\ref{subsec:dataprep-tqa}} to better clarify the connection between the identified error types and the corresponding logical operations proposed in our framework. 


Specifically, as shown in Figure~\ref{fig:error_instance_record}, the majority of TQA errors arise from inadequately addressing three key data prep issues: \emph{missing semantics}, \emph{inconsistent values}, and \emph{irrelevant columns}. To address the challenges, we introduce three types of data prep operations.

%Specifically, this paper considers the following three types of operations.

\bi
	\item \term{Derive}: 
    A data prep task that derives a new column for table $T$ from existing columns, aimed at addressing the challenge of \emph{missing semantics}. This task typically involves operations such as combining columns through arithmetic computations, extracting relevant values, etc.
	\item \term{Normalize}: a data prep task that normalize types or formats of  the values in a column of $T$ based on the needs of $Q$, {aimed at addressing the challenge of \emph{inconsistent values}}. This task typically involves value representation or format normalization, type conversion, etc.
	\item \term{Filter}: A data prep task that filters out columns in $T$ that are not relevant to answer question $Q$, {aimed at addressing the challenge of \emph{irrelevant columns}}.   
    This is crucial for handling large tables to address the input token limitations and challenges in long-context understanding of LLMs~\cite{DBLP:journals/corr/abs-2404-02060}.
\ei

%\revise{We have revised the name of two logical operators and added more description about the connection between our framework and the error analysis in Section XXX.} \lei{check and fix the XXX.} Our three logical operators are designed for the corresponding type of errors. For example, we design \textsc{CellTrans} \fmh{Influence both the revision and the paper.} \lei{what does `influence both the revisio and the paper' mean?}to address the inconsistent data types or formats issues in Cell-Level errors, which make up the vast majority of the Cell-Level errors. We believe that more complicated data quality issues exist in real world scenarios. Thus, \sys is designed based on the Logical-Physical operator implementation, which ensures the extendability of the system to integrate more data prep operations, \eg missing value imputation for \textsc{CellTrans}. 

%\fmh{This has been moved to Appendix.}

\stitle{Impact of missing values and duplication issues in TQA task.} We have conducted a \textbf{new experiment} to analyze the impact of missing values and duplication in TQA tasks on the WikiTQ dataset (our main change \textbf{M\ref{modify:new-exps} (7)}). 

Specifically, for duplication, we first examine all tables containing duplicated records using a heuristic method from~\cite{fan2024cost} on the WikiTQ dataset, and only obtain 24 such instances. Then, we manually remove the duplicate records and re-evaluate \sys’s performance on the updated dataset. The results remain unchanged (accuracy: 70.83\% for both the original and de-duplicated datasets), suggesting that duplication is not a critical issue on existing TQA benchmarking datasets. Similarly, for missing values, we prompt LLMs to impute the missing entries based on the available data for all tables and then re-evaluate \sys on the imputated dataset. The results also show insignificant difference (65.00\% w/o imputation vs. 64.33\% with imputation), indicating that missing values have limited impact.

These above results suggest that such data preparation issues are uncommon and have little effect on existing TQA benchmarking datasets. This is largely due to the way of constructing the datasets. Specifically, during dataset construction~\cite{chen2019tabfact, pasupat2015compositional, wu2024tablebench}, annotators are instructed to first generate natural language questions based on a given table and then derive the corresponding answers directly from the same table. This construction paradigm implicitly ensures data completeness and consistency, as annotators tend to avoid crafting questions around missing or duplicating information. As a result, common data quality issues such as missing values and duplicate records are naturally excluded from the dataset, making them less relevant in the context of existing TQA tasks.

Nevertheless, we acknowledge that issues such as missing values and duplicates are common in real-world datasets. We leave the exploration of these broader data prep challenges to future work.

%Specifically, for duplications, we collect all tables with duplicated records based on a heuristic method from~\cite{fan2024cost} and discover 24 instances from WikiTQ and 0 instance from TabFact in total. Next, we simply remove duplicated records and evaluate \sys’s performance on these instances. Experimental results on duplicated dataset and deduplicated dataset remain the same (Both accuracy are 70.83), which demonstrates that duplicate issue is not critical in TQA task. For missing values, we directly prompt LLMs to predict the missing values based on the available data. The same conclusion has been reached (65.00 without imputation vs 64.33 with imputation). 

%The experimental results indicate that these issues are not common in TQA task. This is because TQA task aims to evaluate LLMs' capabilities of reasoning over table to extract the answer instead of correcting the data itself. In the very beginning of dataset construction for TableQA task, the annotating workers are required to first generate the question based on a given table and then generate the answer based on the question and the original table~\cite{chen2019tabfact, pasupat2015compositional, wu2024tablebench}. Moreover, unlike tables in databases, which are updated in real-time, web-tables crawled from document, paper and internet remain unchanged since constructed. Thus, duplicated values seldom occur in TQA.
%In general, both duplication and missing value issues do not matter much to TQA.
% \lei{Are we arguing these issues rarely occur? Or even if these issues occur, they do not matter much to TQA?}


\begin{shaded}
{
\stitle{R1R2:}
\emph{Add experiments determining whether function pool or custom functions were used and compare their accuracy.}

\stitle{R1D4:} \emph{You use a function pool for specific preparation tasks but for some tasks, which are not covered by the function pool, you use custom LLM-generated code. How often does this happen and how accurate is the custom code compared to the function pool implementations? There are no experiments regarding this aspect.}

}
\end{shaded}



\noindent{\bf RESPONSE}: 
As suggested, we have added a \textbf{new experiment} to evaluate how frequently the custom LLM-generated code is triggered and how accurate it is compared to function pool implementations (our main change \textbf{M\ref{modify:new-exps} (6)}).

Specifically, we quantify the usage frequency of $\mathtt{CustomCode}$ and evaluate whether $\mathtt{CustomCode}$ produces the correct code on WikiTQ.
We also evaluate the performance of \sys without $\mathtt{CustomCode}$ design. 
%
As shown in Table~\ref{tbl:in_response_llm_code_for_op_analysis}, we can see that $\mathtt{CustomCode}$ is invoked in 1.08\% of cases, achieving an accuracy of 55.32\%. Notably, removing $\mathtt{CustomCode}$ leads to a performance drop of \textbf{0.46}  points (from 66.09 to 65.63). These results indicate that, despite its relatively low invocation frequency and moderate accuracy, $\mathtt{CustomCode}$ improves generalization of \sys, particularly in handling new or unforeseen physical operations.

\inresponse{
\input{tables/_in_response_llm_code_for_op_analysis}
}

\stitle{Finding: $\mathtt{CustomCode}$ improves the generalization of \sys on cases requiring new physical implementations.}




%We first generate custom function without using function pool. If fail (\ie, exceeding maximum debugging rounds), we use function pool to generate code again, which we refer to $\mathtt{CustomCode}$ method.

% First, we clarify that given a specific data preparation task, we prioritize using custom functions over the function pool. When no custom function can meet the data preparation needs (\ie, exceeding maximum debugging rounds), we prompt the LLM to generate code to fulfill the data preparation requirements, which we refer to $\mathtt{CustomCode}$ method. \lei{We first generate custom function without using function pool. If fail, we use function pool to generate code again? The above paragraph is not super clear now.}

%We have added \textbf{Exp~\ref{exp:generalization_exp_new_physical_op}} in \textbf{Section~\ref{subsec:evaluation_on_generalization}}. Please refer to \textbf{M\ref{modify:newexp_analyze_custom_code_method}} for more details. In general, $\mathtt{CustomCode}$ \textbf{improves the generalization} of \sys on cases requiring new physical operations.

% \stitle{How often?} As recorded, \sys utilizes $\mathtt{CustomCode}$ in \textbf{1.08\%} cases, indicating that the custom function can cover the absolute majority of cases.

% \stitle{How accurate?} For cases not covered by custom functions (where its accuracy is \textbf{0}), the accuracy of $\mathtt{CustomCode}$ is \textbf{55.32}. This indicates that $\mathtt{CustomCode}$ helps to implement the logical operator when custom functions incur bugs. In future work, we will work on making $\mathtt{CustomCode}$ more reliable.

% \stitle{Ablating $\mathtt{CustomCode}$ from \sys.} Moreover, comparing with \sys equipped only with function pool, \sys with $\mathtt{CustomCode}$ improves the performance on WikiTQ by \textbf{0.46} (from 65.63 to 66.09).

% In summary, the results show that the $\mathtt{CustomCode}$ design in \sys is useful.


\begin{shaded}
{
\stitle{R1R3:} \emph{Add experiments comparing AutoPrep with cleaned data prepared with a regular, offline approach.}

\stitle{R1W3:} 
\emph{Offline preparation as baseline comparison is missing.}

\stitle{R1D11:}
\emph{Even though you conduct thorough experiments, one important baseline is missing in my opinion: data prepared by normal, offline cleaning.}

}
\end{shaded}

\noindent{\bf RESPONSE}:
We have added a \textbf{new experiment} to compare \sys with a new baseline, \textbf{Off-Prep}, which performs \emph{offline} data preparation on all tables in the TQA task (our main change \textbf{M\ref{modify:new-exps} (1)}). 

Specifically, the offline data prep method Off-Prep performs offline data prep operations for all tables in TQA. To this end, we have surveyed and consolidated the offline data prep operations, such as data cleaning, value normalization and column renaming, adopted by current SOTA TQA methods~\cite{yao2022react, cheng2023binding, khot2022decomposed, wang2024chain, DBLP:journals/pvldb/ZhuCXLSZSTL24} to construct a comprehensive offline data prep pipeline, by utilizing the Pandas library~\cite{mckinney-proc-scipy-2010} and the popular DataPrep toolkit~\cite{dataprepeda2021}.

The experimental results are reported in \textbf{Table~\ref{tbl:vs_other_prep_method} of Section~\ref{subsec:Data_Prep_Method_Comparision}}.
\sys improves over Off-Prep by \textbf{10.02} and \textbf{5.55} on average, respectively.  
The performance gap can be attributed to the fact that Off-Prep lacks question guidance, making it ineffective in addressing question-specific issues such as missing semantics and irrelevant columns, as illustrated in Figure~\ref{fig:issue_instances}.
Moreover, predefined normalization routines struggle with table heterogeneity. For instance, standard Pandas normalization cannot handle mixed formats in the \term{Time} column of $T_5$ in Figure~\ref{fig:issue_instances_inconsistency}, whereas \sys can generate specialized code for such cases via LLMs.
%
%Similarly, \sys outperforms ICL-Prep by \textbf{11.00} and \textbf{8.33} on average on the two datasets.  
%This highlights that a well-designed, multi-stage framework is essential for producing comprehensive data prep requirements and precise, executable programs.

\stitle{Finding: \sys significantly outperforms traditional offline data preparation approaches, which validates the necessity of question-aware data prep. 
}

%We have added this baseline in the revised version, as described in \textbf{M\ref{modify:more_baselines}}.
% To construct a offline data prep method, we integrate the offline data prep operations in the current SOTA TQA methods~\cite{cheng2023binding, khot2022decomposed, zhang2024reactable, wang2024chain, DBLP:journals/pvldb/ZhuCXLSZSTL24}. Specifically, It conducts three types of offline data prep operations with Pandas package~\cite{mckinney-proc-scipy-2010} and a popular data prep toolkit DataPrep~\cite{dataprepeda2021}, including (1) column renaming to avoid column misunderstanding and syntax errors in NL2SQL-based Analyzer, e.g., replace “\%” with “percentage”, (2) value cleaning to improve the legibility of the serialized table, e.g., replace “\textbackslash n” with “<br>”, and (3) value normalization to support calculation or comparing operations over tables, e.g., numerical converting and datetime formatting. We have added the above data prep method as \textbf{a new baseline} and update the experimental results in \textbf{Exp~\ref{exp:compare_dataprep_baseline},  Exp~\ref{exp:evaluate_on_tables_with_various_sizes} and Exp~\ref{exp:efficiency_evaluation}}.
%
%\stitle{How does Off-Prep perform?} As shown in Table~\ref{tbl:improve_on_base_TQA_method} and Table~\ref{tbl:vs_other_prep_method}, when comparing with NL2SQL baseline, Off-Prep improves the performance by 2.21 and 7.69 on WikiTQ and TabFact on average. Moreover, as shown in Figure~\ref{fig:accuracy_on_different_size_tables}, when comparing with previous SOTA TQA methods, Off-Prep achieves higher TQA accuracy on cases with large table sizes. The above experimental results indicate the effectiveness of offline data preparation.
%
%\stitle{How does Off-Prep compare to \sys.} However, there still exists a gap on performance between Off-Prep and \sys. Specifically, \sys achieves better performance by 10.02 and 5.55 on WikiTQ and TabFact on average, as shown in Table~\ref{tbl:vs_other_prep_method}. Moreover, \sys outperforms Off-Prep on small, medium and large tables, as illustrated in Figure~\ref{fig:accuracy_on_different_size_tables}. This is because Off-Prep cannot generate precise and customized data prep operations without the guidance of online questions, \eg all missing column issues and redundancy issues in Figure~\ref{fig:issue_instances}. 
%Moreover, a pre-defined data prep program cannot solve all normalization issues. For example, the standard normalization operation in Pandas fails to normalize the column \term{Time} in T5 of Figure~\ref{fig:issue_instances_inconsistency}, which requires utilizing LLMs to generate specific code to convert the string value containing fractions into float. 

%The experimental results above demonstrate the necessity of question-specific data prep and highlight the significance of our proposed Question-Aware Data Prep problem.

\begin{shaded}
{
\stitle{R1R4:} 
\emph{Fix some presentation and wording problems, e.g. position of 2.3 and the use of f(Cyclist).}
}
\end{shaded}
\noindent{\bf RESPONSE}: 
We have already fixed the presentation and wording problems. Please refer to the responses of \textbf{R1D5}, \textbf{R1D6}, \textbf{R1D9}, \textbf{R1D16} and \textbf{R1D17} for more details.

\begin{shaded}
{
\stitle{R1W2:} Exemplars for creating *Analysis Sketch* not explained, even though they might be a big part of the work, since they have to be manually created.
}
\end{shaded}

\noindent{\bf RESPONSE}: 
We clarify that the LLM is prompted to generate an \emph{Analysis Sketch} for each TQA instance, which consists of a structured table and a natural language question.  
As pinpointed by the reviewer, one critical challenge lies in manually creating effective \emph{exemplars} (\ie demonstrations) used in the prompt to guide the generation of the Analysis Sketch. To address this, we follow a systematic process: 

(1) We first select several representative TQA instances from the training set of TQA datasets that involve data prep issues, including missing semantics, inconsistent values and irrelevant columns.  

(2) We filter out redundant cases that exhibit highly similar patterns, \eg two examples both requiring string extraction for column derivation. 

(3) We then manually construct the Analysis Sketches following the syntax specifications outlined in Section~\ref{subsec:planner-cot}.  

To facilitate better understanding, we have included all constructed prompts following the above procedure in the revised version. Due to space constraints, these prompts are provided in
\textbf{
% Figure~\ref{fig:prompt_planner_analysis_sketch_wikitq} and Figure~\ref{fig:prompt_planner_analysis_sketch_tabfact}
Figure 12 and Figure 13
of our technical report~\cite{technical_report}}.

\begin{shaded}
{
\stitle{R1D2:} 
\emph{Is question-aware data preparation really a new problem, or is it simply a form of analysis-specific data cleaning? Especially when considering, that in one of the last steps you transform the natural language query into a SQL statement. The general approach is very similar to normal data preparation for a specific analysis task. }
}
\end{shaded}

\noindent{\bf RESPONSE}: 
We have justified the novelty of question-aware data preparation problem in the \textbf{Introduction} (our main change \textbf{M\ref{modify:problem-novelty}}).

Specifically, the novelty of this problem lies in the need to \emph{deeply understand the semantics of the NL question in order to guide data prep operations over the structured table}. Unlike traditional data prep, which is performed \emph{offline} and independent of downstream tasks, question-aware data prep is conducted \emph{online} and must dynamically tailor the table to the specific demands of the question. This introduces new challenges due to the diversity and ambiguity of NL questions and the heterogeneity of tabular data, requiring precise semantic alignment between the question and the structured table.
%Specifically, the novelty of this problem stems from the fact that TQA requires \emph{semantic alignment between the structured table and the NL question}. Traditional data prep methods typically operate at an {\it offline stage}, independent of any specific downstream question or query. In contrast, question-aware data prep \emph{tailors the tables to the specific needs of the question} during the {\it online stage}, directly addressing the challenge of aligning the table’s structure with the NL question's semantics. 
%
For example, as shown in Figure~\ref{fig:issue_instances_incomplete} in the Introduction, given question $Q_1$ that requests country-specific information from a text column, table $T_1$ needs to be transformed to extract and create a new \term{Country} column, which may not be considered in traditional data prep.

%
%In related work (Section~\ref{sec:related_work}), we have covered more research fields related to ``analysis-specific data cleaning'' and talk about their difference with question-aware data prep. We also update the instances in \textbf{Figure~\ref{fig:issue_instances}} with real and stronger cases to better illustrate the necessity of question-specific data prep. Moreover, we have added a new baseline Off-Prep to highlight the significance of our proposed question-aware data prep method, as explained in \textbf{R3}. 
%
%\stitle{Comparing with other related work.} Machine Learning (ML) oriented Data Preparation is a typical analysis-specific data prep task. It requires generating data prep operations before utilizing an ML model to address a specific analysis task. Thus, the objective of data prep is to improve the prediction accuracy of the ML model. However, for question-aware data prep, the data prep requirement is indistinct, decided by the reasoning process of answering the question 
% \lei{The reasoning process of the question seems weird. the reasoning process of answering the question?}
%and specific data in the table. In addition, our question-aware data prep is different from Data Prep in Exploratory data analysis (EDA), where EDA has no specific question and no data prep requirements. All operations are motivated by the experience and knowledge of data analysts. \lei{Then why do we believe it is relevant?}
% 介绍：where EDA 会进行数据准备操作，一边更好地进行exploratory data analysis，which is an analysis-specific data cleaning
%
%In summary, question-aware data preparation is a new problem that is different from previous analysis-specific data cleaning tasks. Moreover, we confirm that it is a meaningful problem through sufficient experiments and concrete examples.
%
%It is important to note that traditional data prep methods and our question-aware data prep approach are orthogonal: while traditional methods focus on generic data prep, our approach specifically tailors the data to fit the unique requirements of the NL question.


\begin{shaded}
{
\stitle{R1D3:} 
\emph{Page 3: "We implement this AutoPrep architecture with the popular LLM-based Multi-Agent framework, which uses multiple small, independent agents to collaboratively solve complex problems." There is no source following this statement.}
}
\end{shaded}

\noindent{\bf RESPONSE}: Thanks for identifying this issue. 
We have added \textbf{a citation~\cite{han2024llm}} following this statement.
%We have added more discussion on the categories of multi-agent framework in \textbf{Section~\ref{sec:related_work}} and \textbf{cite a paper}~\cite{han2024llm} about the multi-agent framework we refer to. 

\begin{shaded}
{
%
\stitle{R1D5:} 
\emph{Extracting information from a column and putting it in a new column is not data augmentation. Also some of the other examples (concatenate) are not (strictly speaking) data augmentation. Using data extraction or data aggregation would be more precise.}
%
}
\end{shaded}
\noindent{\bf RESPONSE}: 
Thank you for the valuable suggestion.
In the revised version, we have renamed this logical operation to \textbf{Column Derivation}, denoted as \term{Derive}.

We also updated \textbf{Section~\ref{subsec:dataprep-tqa}} to explicitly define \term{Derive} as a data prep task that derives a new column for table $T$ from existing columns, aimed at addressing the challenge of \emph{missing semantics}. This task typically involves operations such as combining columns through arithmetic computations, extracting relevant values, etc.

%\fmh{We plan to name it \textsc{ColumnTrans}.} 


\begin{shaded}
{
\stitle{R1D6:}
\emph{The position within the paper structure of 2.3 is unintuitive. Discussing limitations of existing solutions should come before explaining data prep for TQA, i.e. 2.2.
}
}
\end{shaded}

\noindent{\bf RESPONSE}: 
We would like to clarify that \textbf{Section 2.3} is not intended to discuss the limitations of existing solutions. Instead, it introduces a straightforward LLM-based method for performing question-aware data preparation.

To prevent any potential confusion, we have revised the title of \textbf{Section 2.3} to \textbf{``A Straightforward LLM-based Solution''}.

%Per the suggestion, we have revised the title in \textbf{Section~\ref{subsec:naive_method_for_question_aware_data_prep}} where we introduce a naive LLM-based method of question-aware data prep for TQA problem and its corresponding limitations; we have described the limitation of existing solutions in \textbf{Section~\ref{sec:intro}} (Key Challenge). 

\begin{shaded}
{

\stitle{R1D7}: 
\emph{Is Example 6 derived from a real case or constructed?
}
}
\end{shaded}
\noindent{\bf RESPONSE}: 
Yes, this example is derived from a real case using direct prompting on the WikiTQ dataset. 

%The logical operators are the real output of the direct prompting method.

\begin{shaded}
{
\stitle{R1D8:} 
\emph{
Fig 5 (a): I am somewhat confused. The filter operation states: FILTER([Date, Country, Medal], T) so Cyclist gets filtered out. But Country does not exist. How is filtering defined on not existing columns or does the system assume it is present, i.e. filtering is not done on the actual table columns?}
}
\end{shaded}

\noindent{\bf RESPONSE}: 
We would like to clarify that the \term{Filter} operation retains a nonexistent \term{Country} column simply because the question mentions ``which country.'' However, it fails to recognize that the original table does not actually contain a \term{Country} column. 

This real example clearly illustrates the limitation of the Direct Prompting method. In contrast, our proposed Chain-of-Clauses approach overcomes this limitation by leveraging the analysis sketch, as demonstrated in Figure~\ref{fig:planner-cot}.

%Direct Prompting generates the Filter operation based on the static table and the question. So, it filters \term{Country} because the question asks about the medal number of each country. However, it does not notice that the origin table does not contain column \term{Country}, so the Filter operation is incorrect. In comparison, our Chain-of-Clauses generates the Filter operation based on the Analysis Sketch and other high-level operations and can be adjusted dynamically. Since the analysis sketch contains \term{Cyclist}, \term{Medal} and \term{Date}, it generates an initial Filter operator: \term{Filter}([\term{Cyclist}, \term{Medal}, \term{Date}]). Next, considering \term{Cyclist} is only used to generate column \term{Country}, it removes column \term{Cyclist} and adds a new column \term{Country} to produce the final Filter operator, as shown in Figure~\ref{fig:planner-cot}.

\begin{shaded}
{
\stitle{R1D9}: 
\emph{In 2.1, attributes are labeled $A_n$ and the answer is also labeled A, which is confusing. Moreover, you use f(Cyclist) in the text, but in Fig.5 (b) you use f(T), which is also confusing.
}
}
\end{shaded}

\noindent{\bf RESPONSE}: 
Thanks. We have fixed these issues.

\begin{shaded}
{
\noindent
\stitle{R1D10:} 
\emph{Page 6: "The algorithm generates a Filter operation that only selects columns relevant to the Analysis Sketch." But the Filter operation also adds a new column, right? If so, the name is misleading.
}}
\end{shaded}

\noindent{\bf RESPONSE}: 
No, the \term{Filter} operation removes irrelevant columns, whereas the \term{Derive} operation creates new columns from existing ones, such as via text extraction or mathematical computation. 

We have revised \textbf{Example~\ref{example:cot}} (formerly Example 6) to make this distinction clearer.

%Sorry for the confusion. We clarify that it is \term{Derive} instead of \term{Filter} that adds a new column. The function of \term{Filter} is to select relevant columns from the table with added columns.

\begin{shaded}
{

\stitle{R1D12:} 
\emph{Page 10: "As discussed previously, we evaluate the generalization capabilities of AutoPrep on two TabBench datasets." I was not able to find the previous discussion.
}
}
\end{shaded}

\noindent{\bf RESPONSE}: 
We clarify that the evaluation of generalization capabilities is first introduced when presenting the TabBench dataset in Section~\ref{subsec:exp-setup}. 
%
To improve clarity, we have revised \textbf{Section~\ref{subsec:evaluation_on_generalization}} to explicitly reference this connection.

%We have added some description about the generalization experiment when introducing TabBench. Please refer to \textbf{Section~\ref{subsec:exp-setup}}. 

\begin{shaded}
{

\stitle{R1D13}: 
\emph{Why was AutoTQA mentioned in Related Work, but not used for comparison?
}
}
\end{shaded}

\noindent{\bf RESPONSE}: 
We thank the reviewer for identifying this issue. 
We have conducted a \textbf{new experiment} to compare \sys with a new baseline \textbf{AutoTQA}~\cite{DBLP:journals/pvldb/ZhuCXLSZSTL24}, a SOTA TQA method that also adopts a multi-agent, LLM-based framework (our main change \textbf{M\ref{modify:new-exps} (2)}).

Specifically, the results, shown in \textbf{Table~\ref{tbl:vs_other_prep_method} of Section~\ref{subsec:Data_Prep_Method_Comparision}}, highlight that \sys sets a new SOTA performance on both the WikiTQ and TabFact datasets across LLM backbones. In particular, when compared to AutoTQA, \sys shows significant gains of \textbf{5.81} on WikiTQ and \textbf{2.77} on TabFact. This is because AutoTQA mainly focuses on data analysis, while lacking comprehensive data prep, leading to execution errors or incorrect answers.

The results demonstrate that data prep is inherently complex and cannot be solved with a one-size-fits-all solution. Instead, a more effective strategy involves specialized LLM-based agents for each type of data prep task, coordinated by a centralized planning agent. Moreover, \sys covers a broader range of data prep operations, filling gaps (\eg \term{Derive} and \term{Normalize}) that previous solutions, such as AutoTQA, have not fully addressed.

\stitle{Finding: \sys outperforms \textbf{AutoTQA}, a TQA method that also adopts a multi-agent, LLM-based framework.}

%\stitle{How does \sys compare with AutoTQA?} As shown in Table~\ref{exp:compare_SOTA_TQA_with_prep}, \sys clearly outperforms AutoTQA on WikiTQ and TabFact with different LLM backbones by \textbf{5.71} and \textbf{2.77} on average. Moreover, the overhead of \sys is significantly less than that of AutoTQA. As shown in Figure~\ref{fig:time_money_acc_scatter_map}, \sys achieves better performance than AutoTQA with about $\mathbf{1/35}$ execution time cost and $\mathbf{1/27}$ monetary cost on small tables and $\mathbf{1/44}$ execution time cost and $\mathbf{1/45}$ monetary cost on large tables.

%In summary, the above experiment results confirm that \sys consistently outperform AutoTQA with much less cost.

\begin{shaded}
{
\stitle{R1D14:}
\emph{How is the reusability of code. Even if you describe that analysis targets are mostly heterogeneous, there will be some cases where at least parts of the preprocessing are identical (e.g. the extraction of country). Does this have to be carried out again each time?
}
}
\end{shaded}

\noindent{\bf RESPONSE}:
We agree with the reviewer that when parts of the data preparation process are identical (\eg extracting a country name), the corresponding code can be reused. This observation aligns with our motivation for introducing a function pool in the implementation of physical operations. 

To further clarify this point, we conducted an \textbf{empirical study} on the \textbf{code reusability}, as suggested by the reviewer. Specifically, we measured the number of lines of code generated by the LLM ($Cnt_{LLM}$) and the actual number of lines executed in the final implementation ($Cnt_{Exe}$). We define code reusability as $(Cnt_{Exe} - Cnt_{LLM}) / Cnt_{LLM}$. Based on our records, \sys achieves a code reusability of \textbf{84.96\%} on WikiTQ and \textbf{86.04\%} on TabFact.


%We agree with the reviewer that when parts of the data prep are identical (\eg extraction of country), their code can be reusable. Actually, this motivates us to utilize the function pool in physical op implementation. To further clarify this, we have empirically study the ``\textbf{reusability of code}'' (as mentioned by the reviewer). 
%
%Specifically, we count the number of lines of code generated by the LLM $Cnt_{LLM}$ and the actual number of code lines required to implement the data prep operation $Cnt_{Exe}$. We define the reusability as $(Cnt_{Exe}-Cnt_{LLM})/Cnt_{LLM}$. As recorded, the code reusability of \sys is \textbf{84.96\%} and \textbf{86.04\%} for WikiTQ and TabFact.

% 86.04 for tabfact and 84.96 for WikiTQ
% \stitle{The reusability of code.} To measure the reusability, we counted the number of lines of code generated by the LLM $Cnt_{LLM}$ and the actual number of lines of code required to implement the data preparation operation $Cnt_{Exe}$. We define the reusability as $(Cnt_{Exe}-Cnt_{LLM})/Cnt_{LLM}$. As recorded, the code reusabilities of \sys are \textbf{84.96\%} and \textbf{86.04\%} for WikiTQ and TabFact.

Moreover, even if the custom function itself can be reused, the arguments it requires often vary across tables. For instance, although the data preparation goal, such as extracting country names, may remain consistent, the input formats can differ significantly. Consider two tables: Table A contains values like ``Alej(ESP)'' and ``Dav(ITA)'', while Table B has entries such as ``Alejandro from Spain'' and ``David from Italia''. Despite sharing the same objective, the extraction logic must adapt to these format differences. As a result, it is necessary to regenerate the function arguments for each case to ensure correctness.


%\stitle{Does the code have to be carried out again each time?} Consider that in TQA task, each time the user will provide a question and a \textbf{distinct} table. The same data prep function may require different preparing operations due to the date difference. For example, consider to conduct the ``extracting the country'' operation in two different tables, where TableA contains a column with values ``Alej(ESP)'' and ``Dav(ITA)'' and TableB contains a column with values ``Alejandro from Spain'' and ``David from Italia''. Obviously, although the data prep requirements are the same, the extraction operations on TableA and TableB are different. Thus, we need to generate specific operations to produce the arguments of the custom function each time.

% The design of tool-augmented method ensures high reusability of table processing code, because we only need to clarify the target column and operation on the column and not need to generate codes like iterate over table or capture exceptions. Additionally, we calculate the repetition rate of generated physical operations. Specifically, two physical operations are identical only if they have same physical operation type and same arguments. We find that 23.53\% and 20.22\% physical operations are identical for WikiTQ and TabFact, indicating a potential optimization of physical operation reuse. However, in this paper, we do not consider the reuse design, since it requires semantic matching process among logical operators, which could result in performance drops. We will leave it for future work to design accurate code reusing method. \fmh{I think it is worth to implement a physical operation retrieval module. But we need to add many content about physical operation retrieval in several sections.} % 还是说我们只是把他作为一种展望性的实验？

\begin{shaded}
{
\stitle{R1D15}: 
\emph{Bodensohn et al. show that enterprise data has different characteristics than webtables. Can AutoPrep also be used if, for example, the names of the columns are not meaningful/clear?
}
}
\end{shaded}

\input{plots/tex/accuracy_on_meaningless_columns}

\noindent{\bf RESPONSE}:
% \textbf{(D15)} Yes, \sys can be used for TQA instances with tables containing meaningless column headers. \fmh{new experiement?} 
% \lei{We need to explain why we believe it will work on enterprise data. Otherwise, it is an empty claim. Another way to solve this problem is to claim that in the future, we will evaluate it on enterprise data if there is opportunity.}
Thank you for highlighting this important issue. In response, we have conducted a \textbf{preliminary experiment} in which the column names in WikiTQ are replaced with meaningless identifiers (\eg \term{column\_1}). We then compare the performance of \sys with other TQA methods, and report the results in Figure~\ref{fig:accuracy_on_meaningless_columns}. As expected, the accuracy of all methods decreases, since answering questions over tables with non-descriptive column names is inherently more challenging and demands a combination of table reasoning, data preparation, and deep tabular data understanding. Nevertheless, \sys outperforms the baselines, primarily due to its multi-agent framework that facilitates effective interpretation of table content even when column names are not informative. 

However, we acknowledge that enabling question-aware data preparation over enterprise datasets, such as Spider 2.0~\cite{lei2024spider2}, presents a significantly greater challenge. We plan to systematically investigate this problem as part of our future work.

%Considering that \sys performs excellently in the first two capabilities, it can outperform the existing TQA methods on TQA dataset without meaningful columns.

%To demonstrate it, we have added \textbf{an new experiment} by replacing column names in WikiTQ with meaningless identifiers and compare \sys with other TQA methods. The results are shown in \textbf{Figure xxx}. \fmh{On going... Evaluate on 500 instances: (AutoPrep: 60.60, ReAcTable: 60.20, CoTable: 58.40, Binder: 53.00).}


\begin{shaded}
{

\stitle{R1D16}: 
\emph{In Figure 4, emojis are used for the individual components, which can also be found at the beginning of Chapter 3. This increases recognizability, but they are then no longer used in the rest of the text.}
}
\end{shaded}

\noindent{\bf RESPONSE}: 
Thanks. We have fixed this issue.


\begin{shaded}
{

\stitle{R1D17}: 
\emph{
In some figures (e.g. 3, 4, 6, 9) the font is very small, which makes it difficult to read.}
}
\end{shaded}

\noindent{\bf RESPONSE}: Thanks. We have fixed this issue.



==> response/r2.tex <==
%!TEX root = ../main.tex
\subsection*{Responses to Reviewer \#2}
\label{cover_letter:r2}

\begin{shaded}
{

\stitle{R2W1:}
\emph{The multi-agent framework uses a limited set of tools for data preparation. It is unclear how the system would perform on datasets requiring more complex or diverse data preparation operations.}

\stitle{R2D3:}
\emph{The operations and operators in AutoPrep seem highly tailored to the datasets used in the experiments. It remains unclear how AutoPrep would perform if the required operations for a new dataset extend beyond its current capabilities. Although a generalization evaluation is included, it is uncertain whether the data issues in the evaluated datasets overlap significantly.}

}
\end{shaded}

\noindent{\bf RESPONSE}: 
We thank the reviewer for highlighting this important issue.
In response, we have added a \textbf{new experiment} to evaluate how \sys performs on a dataset that requires new data prep capabilities (our main change \textbf{M\ref{modify:new-exps} (4)}). 

Specifically, we introduce a new type of data prep operation: \textbf{table transformation}, which was extensively studied in the VLDB 2023 Best Paper~\cite{li2023auto}. The goal of table transformation is to convert a non-relational table format into a relational one. As existing TQA benchmark datasets do not consider this type of data prep issue, we construct a new dataset, \textbf{TransTQ}, with the assistance of LLMs. This dataset is publicly available on our GitHub repository. In particular, we prompt an LLM to identify tables from WikiTQ where inverse transformation operations (\eg pivot and stack~\cite{li2023auto}) can be applied, thereby generating non-relational versions of structured tables. These transformed tables replace the originals to evaluate whether \sys can effectively address such data prep challenges, which differ significantly from the column derivation, normalization, and filtering tasks primarily studied in our work.

%Specifically, since no existing TQA benchmarking dataset presents sufficiently complex data quality issues, which has insignificant overlap with the TQA datasets used in our experiments, we construct a \textbf{new dataset TransTQ} with the assistance of LLMs, which is available on our GitHub repository. Specifically, we prompt an LLM to identify tables from WikiTQ where inverse transformation operations (\eg pivot and stack~\cite{li2023auto}) can be applied. These operations are then executed to generate non-relational table formats, introducing new challenges for TQA on \textbf{table transformation}.

As shown in \textbf{Table~\ref{tbl:new_operator_new_operation} of Section~\ref{subsec:evaluation_on_generalization}}, without explicit guidance for handling table transformations, all baseline TQA methods exhibit poor accuracy. In contrast, thanks to the modular design of our multi-agent framework, incorporating a new logical operation (\term{Transform}) requires only minimal human effort, yet significantly boosts \sys's performance to outperform all baselines, \eg outperforming the second-best method by \textbf{9.31} points. Moreover, we also validate that adding this new operation does not degrade the performance of \sys on the original WikiTQ dataset, confirming that its multi-agent architecture is well extensible to support the seamless integration of new data prep functionalities.

\stitle{Finding: \sys demonstrates strong extensibility to the dataset that requires new logical operation types.}


%Specifically, we have constructed \textbf{a new dataset} TransTQ to evaluate how our \sys performs when ``the required operations for a new dataset extend beyond its current capabilities'' and added \textbf{a new experiment} (Exp~\ref{exp:scalability_exp_new_op_type}) in \textbf{Section~\ref{subsec:evaluation_on_generalization}}. Please refer to \textbf{M\ref{modify:newexp_evaluate_generalizability_on_complex_tqa_dataset}} for further details. The results show that AutoPrep demonstrates \textbf{strong generalizability} to datasets that requires new logical operation types.

% Specifically, considering that there is no appropriate TQA dataset with complicated data quality issues we construct a new Dataset TransTQ from WikiTQ with the assistance of LLMs and publish it in our Github Repo. We then evaluate the generalizability of all methods on the new dataset. Firstly, we select a few (\ie two in our experiments) demos from TransTQ and add the demos to the prompts of all methods. Secondly, we evaluate the performance on WikiTQ after integrating new demos.

% \stitle{How does \sys perform?} Without adding new demos, all methods perform poorly on TransTQ. But after integrating the new demos, \sys achieves new SOTA performance comparing with other methods (improve by \textbf{3.25}), as shown in Table~\ref{tbl:new_operator_new_operation}. Moreover, the performance of \sys does not drop on the original WikiTQ dataset. This indicates that our \sys can generalize well on new data quality issues while maintaining its ability on original issues.

% We further evaluate \sys on datasets beyond its capabilities, \eg a dataset requiring complex transforming operations on non-relational tables in Exp~\ref{exp:scalability_exp_new_op_type}. Considering that there is no TQA dataset with complicated data quality issues, we construct a new Dataset TransTQ from WikiTQ with the assistance of LLMs and publish it in our Github Repo. We compare \sys and other TQA methods on TransTQ with or without integrating ICL demonstrations guiding them to generating transforming operations. We do not compare with CoTable since it depends on a predefined finite-state automaton which determines the search space of the operator and is hard to be modified. \textbf{(2) How \sys performs?} As shown in Table~\ref{tbl:new_operator_new_operation}, without specific guidance of ICL demonstrations, all TQA methods perform poorly, especially \sys. However, when integrating guidance of transforming operations, \sys achieves new SOTA performance comparing with other methods. Recall that we do not claim that \sys is comprehensive in solving all data quality issues, but is scalable with the design of logical-physical operators, which is well demonstrated by the results in Exp~\ref{exp:scalability_exp_new_op_type}.


\begin{shaded}
{
\stitle{R2W2}: 
\emph{Several technical aspects, such as the mechanisms for orchestrating operations and converting analyzer sketches into actions, are not adequately explained in the paper.}

\stitle{R2D1:} 
\emph{The order of operations (and operators) that LLMs orchestrate really matters. However, it does not clarify how this order is determined by the planner and programmer.}

\stitle{R2D2:}
\emph{
I am not sure how the analyzer sketch is converted into operations. In particular, it is unclear how LLMs figure out the purpose of each clause and identify the specific columns to manipulate. I try to find the corresponding prompt in the technical report, but it seems not included.
}
%
}
\end{shaded}

\noindent{\bf RESPONSE}: 
Thanks for the suggestion.
In response, we have revised \textbf{Section~\ref{subsec:planner-cot}} to present more technical details on orchestrating operations and converting analyzer sketches into actions. In addition, we have included all the detailed \textbf{LLM prompts}. See our main change \textbf{M\ref{modify:technical-details}}.

First, for orchestrating operations, given the constructed Analysis Sketch, we orchestrate the logical operations and determine their execution order by translating the sketch into actionable steps.
Specifically, we leverage the syntax parser from Binder~\cite{cheng2023binding} to extract all UDFs and operation clauses from the sketch and sort them according to their intended execution sequence from the parser.
Based on this parsed order, we then generate the corresponding logical operations.

%We have revised \textbf{Section~\ref{subsec:planner-cot}}
% \lei{fix the xxx.}
%to clarify the logical operator generation process.
%When we construct the QA-Sketch, we use the syntax parser from Binder~\cite{cheng2023binding} to extract all UDFs and operation clauses in the sketch and sort them by the execution order. Then, we generate the corresponding logical operators based on the parsed executing order.


% We use the method in Binder~\cite{cheng2023binding} to determine the xxx. We have revised Section xxx to clarify this. 
% \sys parses the generated QA-Sketch to determine the order of logical operator. Afterwards, the \textsc{Programmer} generates the physical operations by the order of logical operators. Specifically, the \textsc{Planner} use a syntax parser to extracts all UDFs and operation clauses in the sketch and sort them by the execution order. We have uploaded a running case illustrating how \sys works in Appendix~\ref{sec:appendix_a_running_example_of_autoprep}.

\input{plots/tex/prompt_instance_generating_logical_requirement}

Second, for converting analyzer sketches into actions, we provide several in-context learning demonstrations that guide the LLM to understand the intent of each clause and identify the corresponding data preparation requirements.
%
For better illustration, we provide an example in Figure~\ref{fig:prompt_instance_generating_logical_requirement}. In the prompt, we begin by defining the task through a description and an illustrative example, which includes both the input and the desired output. This helps the LLM understand that the objective is to generate the requirement for a column derivation operation. Next, we present the source columns for analysis and specify that the goal is to derive the column \term{is\_loss} in the Sketch to answer question Q. With this information, the LLM is guided to infer the intent of each clause and identify the corresponding data preparation requirements. Additional details of the prompt construction are provided in our technical report~\cite{technical_report}.

%For better illustration, we provide an example as shown in Figure~\ref{fig:prompt_instance_generating_logical_requirement}. In the prompt, we first define the task by providing the task description and an illustrative example consisting of the input and desired output, from which the LLM can learn the task is to produce the requirement of a column derivation operation. Then, we provide the source columns for the LLM to analyze and remind it that the requirement is to derive the column `is\_loss' in the QA-Sketch to answer question Q. Finally, with all the information provided, the LLM can figure out the purpose of each clause and identify the specific data prep requirements to satisfy.
%We have presented more details of the prompts in our technical report~\cite{technical_report}.

%We have revised \textbf{Section~\ref{subsec:planner-cot}} and added detailed prompts
% (Figure~\ref{fig:prompt_planner_generate_req_aug} and Figure~\ref{fig:prompt_planner_generate_req_norm})
%in our \textbf{Technical Report}.

\begin{shaded}
{
\stitle{R2W3:}
\emph{AutoTQA studies a similar problem, which reportedly achieves better results. A detailed comparison and discussion of the differences between AutoPrep and AutoTQA are necessary.}

\stitle{R2D4:}
\emph{AutoTQA studies a similar problem, which reportedly achieves better performance. The paper does not include a comparative study with AutoTQA, nor does it discuss the key differences between AutoTQA and AutoPrep.}

}
\end{shaded}

\noindent{\bf RESPONSE}: 
Thanks for the suggestion. 
We have added a \textbf{new experiment} to compare with AutoTQA (our main change \textbf{M\ref{modify:new-exps} (2)}), and discussed the differences between AutoPrep and AutoTQA.
The experimental results show that \sys outperforms AutoTQA, which also adopts a multi-agent, LLM-based framework.
Please refer to the response to \textbf{R1D13} for detailed results and analysis. 

%We have added this baseline in the revised version. Please refer to \textbf{M\ref{modify:more_baselines}} for more details and refer to \textbf{R1D13} for the comparison between \sys and AutoTQA.

\begin{shaded}
{
\stitle{R2D5:}
\emph{Discuss the limitations of AutoPrep.}
}
\end{shaded}

\noindent{\bf RESPONSE}: 
We have discussed the limitations of \sys, which provide promising research directions, in the \textbf{Section~\ref{sec:conclusion_and_future_work} Conclusion and Future Work} (our main change \textbf{M\ref{modify:future-work}}). 

First, we aim to extend the system's current data prep capabilities by integrating a broader set of operations to handle more complex issues such as missing values, duplicates, etc. Second, \sys currently focuses on single-table question answering; extending its capabilities to support multi-table TQA is essential for tackling more realistic and complex scenarios.
The third direction is to enable question-aware data preparation over enterprise datasets, which are much more complex than existing TQA benchmarks. 
% enabling question-aware data preparation over enterprise datasets.

%\textbf{Section~\ref{sec:conclusion_and_future_work}}. 

%\stitle{\sys only supports QA on the single table.} In practical scenarios, it is possible that answering a question correctly needs to access the data from different tables. More complicated data quality issues could occur when integrating the tables. For example, how to solve the conflicting fact in two different tables? In addition, data inconsistency issues could occur more frequently, since different tables may come from different sources.
%
%\stitle{\sys only supports QA on the known table.} In open-domain question answering, users will only provide a question and require the system to retrieve relevant data (\eg tables) to answer it. Supporting open QA is one of our future research directions.

%We will extend the capabilities of \sys according to the two limitations above in the future work.










% \begin{shaded}
% {
% \noindent \emph{\underline{R2D1}: 
% % Further explain the order of operation generation.
% D1: The order of operations (and operators) that LLMs orchestrate really matters. However, it does not clarify how this order is determined by the planner and programmer.
% }
% }
% \end{shaded}
% \vspace{-0.5em}
% \noindent{\bf RESPONSE}: \textbf{M\ref{modify:new-exps}-\ref{M\ref{modify:new-exps}:describe_coc}}



% \begin{shaded}
% {
% \noindent \emph{\underline{R2D2}: 
% % Further describe the logical operation generation process
% D2: I am not sure how the analyzer sketch is converted into operations. In particular, it is unclear how LLMs figure out the purpose of each clause and identify the specific columns to manipulate. I try to find the corresponding prompt in the technical report, but it seems not included.
% }
% }
% \end{shaded}
% \vspace{-0.5em}
% \noindent{\bf RESPONSE}: \textbf{M\ref{modify:new-exps}-\ref{M\ref{modify:new-exps}:describe_coc}} 

% We scan the generated QA sketch to extract all operations on columns and supervise LLM with ICL demonstrations to generate logical op. We add the prompt in the technical report.

% % 通过ICL给例子，让大模型直接生成
% % 我们依次扫描qa sketch，某个列上的操作，我们询问LLM给出logical op
% % 添加prompt到technical report


% \begin{shaded}
% {
% \noindent \emph{\underline{R2D3}: 
% % Further generalization evaluation.
% D3: (1) The operations and operators in AutoPrep seem highly tailored to the datasets used in the experiments. It remains unclear how AutoPrep would perform if the required operations for a new dataset extend beyond its current capabilities. (2) Although a generalization evaluation is included, it is uncertain whether the data issues in the evaluated datasets overlap significantly.
% }
% }
% \end{shaded}
% \vspace{-0.5em}
% \noindent{\bf RESPONSE}: We construct a Transform dataset with pivot and stack operators from AutoTable~\cite{li2023auto}. We first utilizing a powerful LLM Deepseek-v3 to select all possible tables to be pivoted or stacked and provide corresponding transforming suggestions. Then, we manually transform the table to a structure not suitable for answering the question. The Transform dataset contains 241 instances in total with 41 stacking instances and 200 pivoting instances. The dataset can be accessed in our Github Repo. We evaluate \sys and other TQA methods which are easy to be integrating to new operations. Notice that we do not compare CoTable~\cite{wang2024chain} because it define a finite state automata to reduce the search space of existing ops. Thus, a new operator Transform can not be plugged in.

% As shown in Table~\ref{tbl:new_operator_new_operation}, after integrating Transform operations, \sys achieves SOTA performance. Moreover, the performance on origin dataset WikiTQ has been improved slightly. \fmh{explain after i analyze the exp result in depth.}

% % First, we define what ``is a new dataset extend beyond its current capabilities''. Since the abilities of \sys is decided by LLM's knowledge and defined operators, the out-of-scope data quality can be categorized as:

% % \begin{itemize}
% %     \item \textbf{Within LLM's knowledge, out of defined operators.}
% %     \item \textbf{Out of LLM's knowledge, within defined operators.} For example, some question will requires domain-specific calculation to generate new columns. The challenges of this problem is to inject the domain knowledge into LLM, which can be solved by continual training or RAG. This is not the focus of our paper.
% %     \item \textbf{Out of LLM's knowledge, Out of defined operators.} To solve this, we need to solve the above two types of questions.
% % \end{itemize}

% % Thus, we need to evaluate \sys on problems within LLM's knowledge, out of defined operators. We design two scenario

% % \sys can be well adapted to this types of problems because: (1) we define two types of operations to solve the problems of incomplete physical operations, i.e., use LLM-generated code for questions failing on defined operations and use LLM prediction for questions can not be solved by code. Refer to R1D4. (2) The Logical-physical design is easy to be extended. We add description of specific extending procedures in the paper. In addition, we design experiment of new operator and new operation, showing that with simple extending effort, \sys improves obviously.

% Seen in Table~\ref{tbl:new_operator_new_operation}

% ``the required operations for a new dataset extend beyond its current capabilities.''

% \input{tables/new_operator_new_operation}

% \begin{shaded}
% {
% \noindent \emph{\underline{R2D4}: 
% % Comparison with AutoTQA
% D4: AutoTQA studies a similar problem, which reportedly achieves better performance. The paper does not include a comparative study with AutoTQA, nor does it discuss the key differences between AutoTQA and AutoPrep.
% }
% }
% \end{shaded}
% \vspace{-0.5em}
% \noindent{\bf RESPONSE}: Compare with AutoTQA.

==> response/r3.tex <==
%!TEX root = ../main.tex
\subsection*{Responses to Reviewer \#3}
\label{cover_letter:r3}

\begin{shaded}
{
\stitle{R3W1:} 
\emph{The proposed approach focus on a limited number of data prep operations, which makes doubtful its generality.}

\stitle{R3D1:}
\emph{The paper focuses on three specific high-level data preparation operations: column augmentation, value normalization, and column filtering. While these are crucial for many TQA tasks, real-world data often presents a broader range of inconsistencies and complexities that the current operations may not address. For instance, the paper doesn't discuss how AutoPrep would handle missing data, erroneous values, or nested data. The paper mentions that the system can be extended to support new tasks, but it does not provide a comprehensive discussion on the practical aspects of adding new operation types.}
}
\end{shaded}

\noindent{\bf RESPONSE}: 
We thank the reviewer for highlighting these important issues.
In response, we first examine the extensibility (\ie the ``generality'' mentioned by the reviewer) of \sys to support new tasks, and then discuss its ability to handle a broader range of data prep issues.

\stitle{Whether \sys can be extended to support new tasks?}
In the revised version, we have added a \textbf{new experiment} (\ie \textbf{Exp-\ref{exp:scalability_exp_new_op_type}}) to evaluate ``\emph{the practical aspects of adding new operation types}'' mentioned by the reviewer (our main change \textbf{M\ref{modify:new-exps} (4)}). 

Specifically, we introduce a new type of data prep operation: \textbf{table transformation}, which was extensively studied in the VLDB 2023 Best Paper~\cite{li2023auto}. The goal of table transformation is to convert a non-relational table format into a relational one. As existing TQA benchmark datasets do not consider this type of data prep issue, we construct a new dataset, \textbf{TransTQ}, with the assistance of LLMs. This dataset is publicly available on our GitHub repository. In particular, we prompt an LLM to identify tables from WikiTQ where inverse transformation operations (\eg pivot and stack~\cite{li2023auto}) can be applied, thereby generating non-relational versions of structured tables. These transformed tables replace the originals to evaluate whether \sys can effectively address such data prep challenges, which differ significantly from the column derivation, normalization, and filtering tasks primarily studied in our work.

As shown in \textbf{Table~\ref{tbl:new_operator_new_operation} of Section~\ref{subsec:evaluation_on_generalization}}, without explicit guidance for handling table transformations, all baseline TQA methods exhibit poor accuracy. In contrast, thanks to the modular design of our multi-agent framework, incorporating a new logical operation (\term{Transform}) requires only minimal human effort, yet significantly boosts \sys's performance to outperform all baselines, \eg outperforming the second-best method by \textbf{9.31} points. Moreover, we also validate that adding this new operation does not degrade the performance of \sys on the original WikiTQ dataset, confirming that its multi-agent architecture is well extensible to support the seamless integration of new data prep functionalities.


\stitle{How \sys handles more data prep issues?}
We agree with the reviewer that the previous version lacked discussion on handling more complex scenarios such as missing data, erroneous values, and nested data. To address this, we have revised \textbf{Section~\ref{subsec:prog-pool}} to discuss these cases. Specifically, the physical operator $\mathtt{infer}$ enables \sys to process values that cannot be handled by standard functions, such as missing or erroneous values. Furthermore, because our Analysis Sketch is defined using SQL-style syntax, which naturally supports querying nested data, we can identify the relevant data prep requirements and apply appropriate operations on the nested structures accordingly.

Moreover, we have conducted a \textbf{new experiment} on the WikiTQ dataset to analyze the impact of missing values and duplicates in TQA tasks (see our main change \textbf{M\ref{modify:new-exps} (7)}). The results indicate that such issues are rare and have minimal impact on current TQA benchmarks, largely due to the controlled construction process of these datasets.
Please see the response of \textbf{R1R1} for more details.

Nevertheless, we acknowledge that issues such as missing values and duplicates are common in real-world datasets. We leave the exploration of these broader data prep challenges to future work (our main change \textbf{M6}).



\begin{shaded}
{
\stitle{R3W2:}
\emph{The paper does not provide details about the generation of the LLM prompts.}

\stitle{R3D2}: 
\emph{The paper omits detailed information about the LLM prompts used in AutoPrep but they are central to the functionality of the system and without the details, it is difficult to assess the validity of the results.}

}
\end{shaded}

\noindent{\bf RESPONSE}: Thanks for the comments. As suggested, we have provided all the detailed \textbf{LLM prompts} used by \sys (our main change \textbf{M\ref{modify:technical-details}}), which are presented in \textbf{Appendix D} of our technical report~\cite{technical_report} due to space limitations.

%in Figures~\ref{fig:prompt_planner_analysis_sketch_wikitq} - \ref{fig:prompt_nl2py_tabfact} in \textbf{Appendix~\ref{appendix:prompts_in_autoprep}}.


\begin{shaded}
{
\stitle{R3W3:}
\emph{While the paper mentions that column filtering can reduce the cost of LLM inference, a more thorough discussion of the computational cost and efficiency of AutoPrep is needed.}

\stitle{R3D3:}
\emph{It is not clear what is the overhead of using a multi agent framework. The paper should include metrics such as processing time, memory usage, and API costs, especially for large tables and complex data preparation operations. In addition, the authors claim that AutoPrep addresses question specific data problems at the online query stage, but there is no discussion on the implications of this design for real-time use.}
}
\end{shaded}

\noindent{\bf RESPONSE}: 
As suggested, we have added a \textbf{new experiment} to evaluat the overhead of \sys in terms of both processing time and API cost, and compared it against baseline methods (our main change \textbf{M\ref{modify:new-exps} (3)}).

The results for both small and large tables are shown in \textbf{Figure~\ref{fig:time_money_acc_scatter_map} of Section~\ref{subsec:efficiency_evaluation}}.
As shown, \sys achieves the best overall performance with insignificant time and monetary costs. Specifically, its cost is lower than all methods except Off-Prep and ICL-Prep. However, \sys significantly outperforms these two baselines in accuracy, achieving improvements of at least \textbf{9.36} and \textbf{5.77} points on small and large tables, respectively. Furthermore, as table size increases, \sys maintains a much more stable time and cost overhead compared to other state-of-the-art TQA methods.
This efficiency stems from the program-based data prep mechanism of \sys, which avoids high latency and API expenses associated with directly processing tables via LLMs. For instance, in the column derivation task on Table $T_1$ (Figure~\ref{fig:issue_instances_incomplete}), CoTable invokes LLMs to generate a full list of country codes. In contrast, \sys only generates a physical operator $\mathtt{extract}$ and executes it to produce the column, which results in significantly lower time and monetary costs, particularly on large tables.

\stitle{Finding: 
\sys achieves the best accuracy with lower cost across varying table sizes, highlighting its practicality for real-time use.
}

%We have added \textbf{a new experiment} to evaluate the efficiency of \sys and other methods in \textbf{Exp~\ref{exp:efficiency_evaluation}}. Please refer to \textbf{M\ref{modify:newexp_overhead_comparison}} for more details.

%except two data prep baselines
%\stitle{How efficient is \sys?} As shown in Figure~\ref{fig:time_money_acc_scatter_map}, \sys achieves the \textbf{best} performance with \textbf{less} time and monetary cost than all TQA methods. Moreover, the overhead of \sys remains stable when varying the sizes of the tables. This is because all data prep operations in \sys are conducted by programs, avoiding the substantial time costs and financial expenses associated with directly processing tables with LLMs. 

%\stitle{Using \sys online.} The average execution time to answer a question with \sys is \textbf{6.07s} and \textbf{7.35s} on small and large tables, and the average monetary cost is \textbf{\$0.0013} and \textbf{\$0.0014}. Therefore, the high efficiency of \sys well supports real-time use.
% \begin{shaded}
% {
% \noindent \emph{\underline{R3D1}: 
% % Describe the opportunity of using \sys for new data prep task, i.e., missing data, erroneous values and nested data. Moreover, describe how can we add a new type of logical operator for \sys?
% D1(W1): The paper focuses on three specific high-level data preparation operations: column derivation, value normalization, and column filtering. While these are crucial for many TQA tasks, real-world data often presents a broader range of inconsistencies and complexities that the current operations may not address. For instance, the paper doesn't discuss how AutoPrep would handle missing data, erroneous values, or nested data. The paper mentions that the system can be extended to support new tasks, but it does not provide a comprehensive discussion on the practical aspects of adding new operation types.
% }
% }
% \end{shaded}
% \vspace{-0.5em}
% \noindent{\bf RESPONSE}: See in R2D3.


% \begin{shaded}
% {
% \noindent \emph{\underline{R3D2}: 
% % Request for detailed information of prompts in technical report.
% D2 (W2): The paper omits detailed information about the LLM prompts used in AutoPrep but they are central to the functionality of the system and without the details, it is difficult to assess the validity of the results.
% }
% }
% \end{shaded}
% \vspace{-0.5em}
% \noindent{\bf RESPONSE}: See in R2D2.


% \begin{shaded}
% {
% \noindent \emph{\underline{R3D3}: 
% % Discuss the computation overhead such as processing time, memory usage, and API costs, especially for large tables and complex data preparation operations. Moreover, talk about practical application of \sys.
% D3(W3): It is not clear what is the overhead of using a multi agent framework. The paper should include metrics such as processing time, memory usage, and API costs, especially for large tables and complex data preparation operations. In addition, the authors claim that AutoPrep addresses question specific data problems at the online query stage, but there is no discussion on the implications of this design for real-time use.
% }
% }
% \end{shaded}
% \vspace{-0.5em}
% \noindent{\bf RESPONSE}: Seen in Figure~\ref{fig:time_money_acc_scatter_map}

% \input{plots/tex/time_money_acc_scatter_map}

==> secs/experiment.tex <==
%!TEX root = ../main.tex
\section{Experiments}
\label{sec:exp}

This section evaluates our batch prompting framework \sys investigated in this paper.
%Specifically, we first present the experimental setup, and then conduct experiments to evaluate \sys.
%answer the following key questions:

% \stitle{Exp-1:} How does \emph{Batch Prompting} compare with \emph{Standard Prompting}? (Section~\ref{subsec:exp-batch-vs-standard})

% \stitle{Exp-2:} What are effective strategies in our design space of question batching and demonstration selection? (Section~\ref{subsec:exp-design-space})

% \stitle{Exp-3:} How does our proposed \sys framework compare with PLM-based approaches to ER? (Section~\ref{subsec:exp-compare-plms})

% \stitle{Exp-4:} How does our proposed \sys framework compare with LLM-based approaches to ER? (Section~\ref{subsec:exp-compare-llms})

% \stitle{Exp-5:} What is performance of our \sys framework given various underlying LLMs? (Section~\ref{subsec:exp-given-llms})

% \stitle{Exp-6:} What is performance of our \sys framework given different feature extractors? (Section~\ref{subsec:exp-given-feat-extract})

% \add{\stitle{Exp-7:} Is it feasible to substitute the use of crowd workers with API requests to Large Language Models(LLMs) as a cost-effective alternative? (Section~\ref{subsec:exp-LLM-labeler})}

\input{secs/exp-setup}
\input{secs/exp-batch-vs-standard}
\input{secs/exp-design-space}
\input{secs/exp-compare-plms}
\input{secs/exp-compare-llms}
\input{secs/exp-hyper-parameters}
\input{secs/exp-LLM-labeler}


==> secs/experiment/07case_study.tex <==
\subsection{Case Studies}
\label{subsec:case_study}

\input{figures/tex/case_study}

%Based on the experimental results, \sys outperforms the two most powerful TQA methods ReAcTable and CoTable. 

This section presents two illustrative examples from TabBench and WikiTQ to qualitatively analyze effectiveness of \sys. 

To answer the question in Figure~\ref{fig:case_study1}, CoTable generates an operator chain with an ``add\_col'' operator, which is used to generate a new column \term{Tol} based on the division results of two existing columns \term{Expense} and \term{Percent}. This operator directly prompts an LLM to output a list containing all values of the new column, which is a challenging task for previous LLMs. Thus, CoTable generates a new column with two wrong values which leads to a wrong answer. For ReAcTable, although it generates a logically correct Python program, it ignores the types of existing columns which do not support for numerical calculation. Thus, ReAcTable also fails to derive the \term{Tol} column.
\sys addresses this issue by first utilizing a \textsc{Planner} agent to generate logical operators specifying data prep requirements, i.e., two $\mathtt{Normalize}$ to normalize column \term{Expense} and \term{Percent}, a $\mathtt{Derive}$ to generate the overall expenses \term{Tol} and a $\mathtt{Filter}$ to select related columns \term{Year} and \term{Tol}. 
These logical operators are passed to \textsc{Programmer} agents to generate physical operators consisting of a pre-defined Python function. For example, we call $\mathtt{to\mbox{-}numerical}$ function two times to cast \term{Expense} and \term{Percent} to numerical values.
All physical operators are executed to process the original table and output a prepared table. Finally, an \textsc{Analyzer} agent based on NL2SQL method generates a SQL query to extract the correct answer ``4214.17''.


Figure~\ref{fig:case_study2} illustrates a TQA instance involving large tables and inconsistent values. 
%To answer the question, CoTable selects all relevant rows for the question. However, it loses related information due to the maximum input token limitation. Specifically, the table is cropped to include only the first 100 rows to fit within the prompt. Thus, all data in the last 103 rows is lost. Consequently, it generates a sub-table table with incomplete data, resulting in an incorrect answer ``3''. For ReAcTable, it reacts in multiple steps to process the table. When filtering records with \term{Date} after ``november 15, 2007'', it does not transform the \term{Date} into comparable format before using operator ``$>$'' to filter the records. Thus, ReAcTable also generates an error answer.
\sys solves this by splitting the TQA question into two phases, i.e., data prep and data analysis. It first generates logical operators including two $\mathtt{Normalize}$ and one $\mathtt{Filter}$. Next, the \textsc{Programmer} agents implement them with corresponding physical operators, which are executed to produce a prepared table. Based on this, the \textsc{Analyzer} agent extracts the final answer ``8''.




==> secs/experiment/07error_analysis.tex <==
\revise{
\input{plots/tex/subcategories_in_other}

\subsection{Details of Error Analysis}
\label{subsec:details_of_error_analysis}
This section presents details of the error analysis shown in Figure~\ref{fig:error_instance_record}, which motivates us to study question-aware data prep.

\stitle{TQA Method: NL2SQL Based on GPT-4.}
We adopt NL2SQL~\cite{rajkumar2022evaluating}, a representative TQA baseline that does not perform data prep, as introduced in Section~\ref{subsec:exp-setup}. Specifically, given a natural language question $Q$ and a table $T$, we prompt GPT-4 to generate an SQL query $\term{SQL}$ using a few-shot in-context learning strategy. The query is then executed on $T$ to obtain the final answer $A$ for $Q$.

\stitle{Error Categorization.}
We recruite three graduate students from our university's database group to annotate error categories for a randomly sampled set of 500 instances from WikiTQ and TabFact. All annotators have a good understanding of the TQA task and are proficient in SQL syntax.
%
We instruct the annotators to first identify errors stemming from insufficient data prep, assigning any remaining errors to a default category labeled \term{Other}. For the data prep-related errors, after careful investigation, we further categorize them into the following three types:
(1) \textbf{Missing Semantics:} The table lacks necessary semantic information required to accurately answer the NL question. 
(2) \textbf{Inconsistent Values:} Values within a column are represented inconsistently across different records. 
(3) \textbf{Irrelevant Columns:} The table includes many columns, but only a small subset are actually relevant to the NL question. 
%
%We introduce the details of error analysis in Figure~\ref{fig:error_instance_record} regarding the TQA method, classification criteria for errors, and labeling. We also introduce the sub-categories in ``Other'' category.
%
%\stitle{The TQA Method: NL2SQL based on GPT4.} Consider a question $Q$, and a table $T$. We first prompt a powerful LLM GPT4 with the serialized table and the question to generate an SQL query $\term{SQL}$ with the supervision of few-shot In-Context Learning demonstrations. Then, we extract the answer $A$ of $Q$ by executing $\term{SQL}$ on $T$.
% The prompt of this NL2SQL based TQA method is shown in Figure~\ref{fig:prompt_nl2sql_wikitq}.

%\stitle{Classification Criteria for Error Categories.} We mainly focus on errors caused by the insufficient data prep and categorize errors that are not related to data prep into other categories. For data prep related cases, the error types are extracted into three categories manually based on whether the data prep operation required is on the cell (Cell-Level), the column (Column-Level), or the entire table (Table-Level) as shown in the Figure~\ref{fig:issue_instances}.
%
%\stitle{Labeling.} We hire 3 graduate students from the database group in our university to conduct error category labeling for the sampled 500 instances from WikiTQ and TabFact. All students are familiar with the TQA task and SQL syntax.

% \subsection{Error Cases in ``Other''  Category}



\stitle{In-depth Analysis of the ``\term{Other}'' Category}. 
We report the detailed sub-categories within the ``\term{Other}'' category in Figure~\ref{fig:subcategories_in_other}. As shown, for WikiTQ, more than half of the cases stem from issues inherent to the dataset itself. Notably, 40\% of the errors are due to limitations in the evaluation function, where semantically equivalent but non-identical responses are marked as incorrect, a problem also highlighted in~\cite{cheng2023binding}. Additionally, 20\% of the errors arise from formatting issues in the model’s responses, where the generated SQL logic is correct but the output includes extraneous values from irrelevant columns.
%
On the other hand, for the TabFact dataset, most errors are attributed to model reasoning failures. Over 50\% result from the model’s inability to generate logically complete and accurate SQL queries. Furthermore, more than 35\% of the errors are due to response formatting issues, where the model returns ambiguous values instead of definitive true/false answers. 



%We report the detailed sub-categories in ``Other'' in Figure~\ref{fig:subcategories_in_other}. As shown in the figure, for the "Other" category in WikiTQ, more than half of the cases are attributed to issues related to the inherent quality of the dataset itself. Specifically, 40\% of the errors arise from an incomplete evaluation function. This finding is also observed in~\cite{cheng2023binding}, where semantically equivalent but not entirely identical responses are deemed mismatched. Additionally, 20\% of the examples result from incorrect formatting in the model's responses, where the SQL logic is correct but the execution results include values from columns other than those required by the answer. In the TabFact dataset, the majority of errors stem from failures in model reasoning. Specifically, over 50\% of the errors are caused by the model's inability to generate comprehensive and logically correct SQL queries. Furthermore, more than 35\% of the errors are due to the model producing responses in incorrect formats. In some cases, the model erroneously extracts certain values, failing to provide a definitive true or false response. We give real examples to further describe each sub-categories in our technical report.

% \input{tables/wikitq_evaluation_error}
% \input{tables/wikitq_labeling_error}
% \input{tables/wikitq_unclear_question}
% \input{tables/wikitq_value_retrieval_error}
% \input{tables/wikitq_answer_format_error}

% \input{tables/tabfact_unclear_question}
% \input{tables/tabfact_reasoning_error}
% \input{tables/tabfact_answer_format_error}

% \stitle{Specific Cases in Subcategories.} We now delve into specific cases within each subcategory to provide a clearer understanding of the ``Other'' category in WikiTQ and TabFact. We provide the TQA instance, generated SQL, predicted results and reason why the prediction is wrong for each subcategories in WikiTQ and TabFact, as illustrated in Table~\ref{tbl:wikitq_evaluation_error}, Table~\ref{tbl:wikitq_labeling_error}, Table~\ref{tbl:wikitq_unclear_question}, Table~\ref{tbl:wikitq_value_retrieval_error}, Table~\ref{tbl:wikitq_answer_format_error}, Table~\ref{tbl:tabfact_unclear_question}, Table~\ref{tbl:tabfact_reasoning_error} and Table~\ref{tbl:tabfact_answer_format_error}.

}

==> secs/related_work.tex <==
%!TEX root = ../main.tex
\section{Related Work} 
\label{sec:related_work} 

\noindent \textbf{PLM-based Methods for Entity Resolution.}
Entity resolution is a popular data integration task that has been widely studied for decades. 
%Previously,  a number of solutions have been proposed leveraging rules~\cite{DBLP:conf/vldb/ChaudhuriCGK07, DBLP:journals/pvldb/FanJLM09},   traditional machine learning methods~\cite{DBLP:journals/pvldb/WangLYF11, DBLP:conf/kdd/BilenkoM03} and crowdsourcing~\cite{wang2012crowder, DBLP:conf/sigmod/ChaiLLDF16} etc. 
With the rise of deep learning, some approaches~\cite{DBLP:journals/pvldb/EbraheemTJOT18} leverage pre-trained word embeddings to improve the ER performance. However, these methods mainly use the non-contextual embeddings without considering the downstream tasks. Therefore, recent studies~\cite{ditto, jointbert, tu2023unicorn, tu2022domain} have focused on using Transformer-based PLMs to produce contextualized embeddings based on fine-tuning over downstream tasks. To be specific, Ditto~\cite{ditto} regards ER as a sequence-pair classification problem via Transformer, where domain knowledge  is injected to further improve the performance. 
% JointBERT~\cite{jointbert} adopts a dual-objective training  paradigm for BERT. Specifically, besides predicting matching/non-matching pairs, JointBERT also incorporates a multi-class classification task to predict the entity identifier for each entity description of a pair. 
DADER~\cite{tu2022domain} focuses on leveraging the domain adaptation technique: given a labeled source dataset, it trains an ER model for another target dataset by aligning features of both datasets based on PLMs. Based on PLMs, Unicorn~\cite{tu2023unicorn} focuses on building a unified framework for data matching tasks, including ER. Unicorn uses a unified encoder for any pair of data to be predicted, and a mixture-of-experts module to align the semantics of multiple tasks. Although the above PLMs-based approaches can achieve a relatively good performance, they need plenty of labeled pairs for supervision, which are often expensive to acquire.

\stitle{LLM-based Methods for Entity Resolution.} 
With the size of pre-training data and model parameters scales, large-scale language models (LLMs) have gained an emergent capability called In-Context Learning (ICL) to learn from a few \demos without explicit model update~\cite{DBLP:conf/nips/BrownMRSKDNSSAA20, chowdhery2022palm}. 
Recent studies~\cite{DBLP:journals/pvldb/NarayanCOR22,DBLP:journals/corr/abs-2310-11244,zhang2023large} have focused on utilizing the LLMs to tackle ER with less labeled pairs for supervision. Narayan et al.~\cite{DBLP:journals/pvldb/NarayanCOR22} are among the first to explore the capability of GPT-3~\cite{DBLP:conf/nips/BrownMRSKDNSSAA20} for ER with manually designed \demos, which achieves remarkable performance compared with PLM-based methods. Since manual \demos require professional prompting engineering knowledge, Peeters et al.~\cite{DBLP:journals/corr/abs-2310-11244} propose to select relevant \demos based on $k$NN retrieval algorithm, where Jaccard similarity is utilized to measure the relevance. Moreover, Zhang et al.~\cite{zhang2023large} consider batch prompting for ER, which employs a straightforward random batching strategy with manually designed demonstrations.
Although question batching and demonstration selection have been considered in existing studies, these studies mainly rely on domain experts or develop heuristics for these two problem, and have not explored the combination of different demonstration selection and batching strategies. Compared to them, we utilize the power of ICL and propose a comprehensive framework \sys. We explore a design space to evaluate the performance of different design choices, and propose a covering-based demonstration selection strategy that effectively balances the trade-off between accuracy and cost.

\stitle{In-Context Learning for Data Management.} LLMs are capable to capture rich linguistic patterns and generate coherent text~\cite{agrawal2022large, DBLP:conf/nips/BrownMRSKDNSSAA20, touvron2023llama}, which have shown great success in a wide range of NLP tasks ~\cite{wan2023gptre, agrawal2022context,li2023unified}.
ICL is an emergent capability of LLMs that enables the model to learn from few demonstrations without explicit gradient update~\cite{chowdhery2022palm}. Recently, researchers have studied to leverage ICL to solve data management tasks, such as data discovery~\cite{DBLP:journals/corr/abs-2306-09610}, data cleaning and integration~\cite{DBLP:journals/pvldb/NarayanCOR22}, and data labeling~\cite{DBLP:journals/corr/abs-2311-00739}, and also study how to batch questions and select demonstrations. BatchPrompt~\cite{cheng2023batch} proposes to group multiple questions into one batch and query LLMs to answer one batch in an interface. In addition, both relevance-based~\cite{DBLP:conf/acl-deelio/LiuSZDCC22, DBLP:conf/coling/LeeLC22} and diversity-based~\cite{DBLP:conf/acl/LevyBB23, DBLP:conf/iclr/SuKWSWX0OZS023} strategies are proposed for demonstration selection.
Compared with these studies, as far as we know, we are the first to develop the batch prompting technique tailored to the ER task, and design new methods, such as covering-based demonstration selection and structure-aware feature extraction, which are shown to be effective for ER.

%have focused on utilizing LLMs to tackle Entity Resolution task in a generative manner. 
%In this era, demonstration selection plays a significant role in the effect of ICL. Specifically, researchers design manually demonstrations or develop heuristic methods to select beneficial demonstrations. In the former category, Narayan et al.~\cite{DBLP:journals/pvldb/NarayanCOR22} utilize GPT3 for data management task by manually designing 10 demonstrations for each dataset, which requires professional prompting engineering knowledge. While the latter category, instead of using manual demonstration, researchers propose to automatically select relevant demonstrations and label it afterwards to improve performance. Peeters et al.~\cite{DBLP:journals/corr/abs-2310-11244} select relevant demonstrations based on $\mathtt{KNN}$ retrieval algorithm, which utilizes Jaccard similarity function to calculate the relevance among data points and reteieve topk most relevant demonstrations for each question. Although it is demonstrated that relevant demonstrations help to improve the performance, they do not consider the annotation cost for labelling these demonstrations. What's more, these methods are all based on Standard prompting, which bring high cost for interfacing LLMs. To reduce the cost, Batch Prompting~\cite{cheng2023batch} proposes to group multiple questions into one batch and query LLMs to answer one batch at one interface. Zhang et al.~\cite{zhang2023large} first evaluate Batch Prompting on ER task, which uses random batching and cluster batching along with manually designed demonstrations. Despite that Batch Prompting can obviously reduce interfacing cost while maintaining performance, previous works have not explored the combination of different demonstration selection and batching strategies. 
%
%Compared to these works, we utilize the power of In-Context Learning and propose a framework for Batch Prompting. We explore a design space to comprehensively evaluate the performance of different Batch Prompting methods. Also, we propose a covering-based demonstration selection strategy that achieves effective trade-off between accuracy and cost.

%\noindent \textbf{In-context learning for data management.} %LLMs are capable to capture rich linguistic patterns and generate coherent text ~\cite{agrawal2022large, gpt3, touvron2023llama}, which have shown great success in a wide range of NLP tasks ~\cite{wan2023gptre, agrawal2022context, rubin2021learning, li2023unified}. 
%Recently, researchers have studied to leverage ICL to solve data management tasks, like data discovery~\cite{DBLP:journals/corr/abs-2306-09610}, data cleaning and integration~\cite{DBLP:journals/pvldb/NarayanCOR22}, data labeling~\cite{DBLP:journals/corr/abs-2311-00739}, etc.


%\fmh{Original In-context learning for data management: }
%\noindent \textbf{In-context learning for data management.} %LLMs are capable to capture rich linguistic patterns and generate coherent text ~\cite{agrawal2022large, gpt3, touvron2023llama}, which have shown great success in a wide range of NLP tasks ~\cite{wan2023gptre, agrawal2022context, rubin2021learning, li2023unified}. 
%ICL is an emergent capability of LLMs that enables the model to learn from few demonstrations  without explicit gradient update~\cite{brown2020language, chowdhery2022palm}. Recently, researchers have studied to leverage ICL to solve data management tasks, like data discovery~\cite{DBLP:journals/corr/abs-2306-09610}, data cleaning and integration~\cite{DBLP:journals/pvldb/NarayanCOR22}, data labeling~\cite{DBLP:journals/corr/abs-2311-00739}, etc. For example, Narayan et al.~\cite{DBLP:journals/pvldb/NarayanCOR22} is among the first to explore the capability of GPT3 ~\cite{gpt3} in tackling ER task. With manually design demonstrations, GPT3 can achieve remarkable performance compared with PLM-based methods. 
%A closer work~\cite{robem} to us that  is yet to go through the peer review process \cc{leverages  model-based entity matching systems in real-world scenarios with different data distributions, identifying data imbalance as a critical issue and proposing simple yet effective modifications to enhance model reliability and outperform existing state-of-the-art solutions.}
%
%\cc{The below things about ICL can be considered to merge with the above paragraph.}

%
% In the era of ICL, demonstration selection plays a significant role in the effect of ICL. At a high level, heuristic~\cite{}  and LLM-based~\cite{} approaches are two main categories for demonstration selection. In the former category, $k$NN based retreiver~\cite{DBLP:conf/acl-deelio/LiuSZDCC22, DBLP:conf/coling/LeeLC22} is leveraged to select demonstrations that are semantically relevant to the query. But this strategy conducts  the selection individually for each demonstration, rather than considering the demonstration set as a whole. 
%To address this, diversity-based strategies~\cite{DBLP:conf/acl/LevyBB23, DBLP:conf/iclr/SuKWSWX0OZS023} are proposed top select the most representative  demonstrations customized to each task.
%\cc{We consider both?}
%The latter category uses the LLMs to select demonstrations. For instance, LLMs can be directly used to measure the demonstration utility based on the performance improvement after the demonstration is added~\cite{DBLP:journals/corr/abs-2302-13539}. Also, EPR~\cite{DBLP:conf/naacl/RubinHB22} first retrieves some semantically similar demonstrations and rank them based on a model trained with examples labeled by LLMs. Besides, the demonstration format~\cite{DBLP:journals/csur/LiuYFJHN23, DBLP:journals/corr/abs-2210-11416, DBLP:conf/nips/Wei0SBIXCLZ22} and order~\cite{DBLP:conf/icml/ZhaoWFK021, DBLP:conf/acl-deelio/LiuSZDCC22} are also important to the performance of ICL.




==> tables/_in_response_llm_code_for_op_analysis.tex <==
\begin{table}[t]
    \centering
    \caption{\bf{Analyzing LLM generated code for logical operator.}}
    \label{tbl:in_response_llm_code_for_op_analysis}
    \vspace{-0.5em}
    \resizebox{0.65\linewidth}{!}{
    \begin{tabular}{|c||c|}
        \hline
        \textbf{Method} & ~\textbf{WikiTQ}~  \\ \hline \hline
        $\mathtt{CustomCode}$ ratio & ${1.08\%}$  \\ \hline
        $\mathtt{CustomCode}$ accuracy & ${55.32\%}$ \\ \hline \hline
        
        \sys w. $\mathtt{CustomCode}$ & $\textbf{66.09}$\\ \hline
        \sys w.o. $\mathtt{CustomCode}$ & ${65.63}$  \\ 
        \hline
    \end{tabular}
    }
    \vspace{-1em}
\end{table}


% 47 个case调用$\mathtt{CustomCode}$


==> tables/_in_response_mainexp_compare_autoprep_with_new_baselines.tex <==
%!TEX root = ../main.tex
\begin{table*}[t]
  \centering
  \caption{\bf{{Compare \sys with new baselines.}}
  }
  \vspace{-0.5em}
  %\vspace{-1em}
  % \renewcommand{\arraystretch}{1.2}
  % \tabcolsep=0.11cm
\resizebox{0.87\linewidth}{!}{
    \begin{tabular}{|c||c|c|c|c|c|c|c|c|}
      \hline
      \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c|}{\textbf{DeepSeek}} & \multicolumn{2}{c|}{\textbf{GPT3.5}} & \multicolumn{2}{c|}{\textbf{Llama3}} & \multicolumn{2}{c|}{\textbf{QWen2.5}} \\ \cline{2-9}
                                                      & \textbf{~WikiTQ~}                                                       & \textbf{~TabFact~}                                                       & \textbf{~WikiTQ~}                                                       & \textbf{~TabFact~}                                                       & \textbf{~WikiTQ~}                                                        & \textbf{~TabFact~}                                                      & \textbf{~WikiTQ~}                                                        & \textbf{~TabFact~}                                                      \\
      \hline \hline
		{Off-Prep}  & {${55.32}$}       & {$81.67$}          & {$56.86$}         & {$\underline{81.52}$}          & {$53.02$}         & {$75.40$}          & {$58.01$}         & {$82.31$}          \\ \cline{1-9} % [1pt]
		{AutoTQA*}  & {${60.80}$}       & {$84.40$}          & {$58.40$}         & {$80.60$}          & {$58.80$}         & {$82.40$}          & {$62.40$}         & {${83.00}$}          \\ \cline{1-9} % [1pt]
      \hline \hline
	 {\sys}     & $\textbf{66.09}$       & $\textbf{87.85}$        & $\textbf{64.75}$       & $\textbf{84.19}$        & $\textbf{63.72}$       & $\textbf{85.72}$        & $\textbf{68.72}$       & $\textbf{85.33}$          \\
      \hline
    \end{tabular}
  }
  \label{tbl:_in_response_vs_other_prep_method}
  % \vspace{-1em}
\end{table*}

==> tables/_in_response_new_operator_new_operation.tex <==
\begin{table}[t]
  \centering
  \caption{\bf{
        Evaluating generalization on dataset requiring new operator type.
    }}
  \vspace{-0.5em}
  \resizebox{0.7\linewidth}{!}{
    \begin{tabular}{|c||c|c|c|}
      \hline
      \multirow{2}{*}{\textbf{Method}}  & \multirow{2}{*}{\textbf{TransTQ}}  & \multicolumn{2}{c|}{\textbf{WikiTQ}} \\ \cline{3-4}
               &  & \textbf{~origin~} & \textbf{~after~}  \\
      \hline \hline
      ICL-Prep  & 58.92             & 56.54             & 55.00             \\ \cline{1-4} % [1pt]
      ReAcTable  & 51.04             & \underline{64.13} & \underline{63.03} \\ \cline{1-4} % [1pt]
      AutoTQA       & \underline{59.75} & 60.80             & 61.20             \\
      \hline \hline
      \sys        & \textbf{68.88}    & \textbf{66.09}    & \textbf{66.28}    \\ \hline
    \end{tabular}
  }
  \label{tbl:_in_response_new_operator_new_operation}
  % \vspace{-1em}
\end{table}

==> tables/ablation_exp.tex <==
\begin{table}[t!]
  \centering
  \caption{\bf{Ablation Study of \sys.}}
  % \tabcolsep=0.45cm
%  \renewcommand{\arraystretch}{1.15}
   \vspace{-0.5em}
  \begin{tabular}{|c||c|c|c|}
    \hline
    \textbf{Method} & ~\textbf{WikiTQ}~                                          & ~\textbf{TabFact}~        & { ~\textbf{TabBench}~}                                         \\ \hline \hline
    \sys   & $\textbf{66.09}$                                                    & $\textbf{87.85}$    													& { $\textbf{50.10}$}                                                    \\ \hline \hline
    - Filter\qquad\qquad     & $62.78$ {\scriptsize \textcolor{dropred}{($-3.31$)}}     & $84.98$  {\scriptsize \textcolor{dropred}{($-2.87$)}}           & {$47.67$} {\scriptsize \textcolor{dropred}{($-2.43$)}}                                       \\ \hline
    ~~- Derive      & $61.79$ {\scriptsize \textcolor{dropred}{${(-4.30)}$}}          &   $85.67$ {\scriptsize \textcolor{dropred}{($-2.18$)}}           & {$45.44$} {\scriptsize \textcolor{dropred}{($-4.66$)}}                                                    \\ \hline
    ~~- Normalize      & $62.02$  {\scriptsize \textcolor{dropred}{($-4.07$)}}         &  $83.79$ {\scriptsize \textcolor{dropred}{${(-4.06)}$}}              & {$41.58$} {\scriptsize \textcolor{dropred}{${(-8.52)}$}}                                                  \\    \hline 

  \end{tabular}
  \label{tbl:ablation_exp}
  \vspace{-0.5em}
\end{table}

==> tables/different_analyzer.tex <==
%!TEX root = ../main.tex

\begin{table}[t!]
	\centering
	\caption{\bf{Impact of data prep on TQA Methods.}}
	% \tabcolsep=0.4cm
%	\renewcommand{\arraystretch}{1.12}
   \vspace{-0.5em}
	\begin{tabular}{|c||c|c|}
		\hline
		\textbf{Method} & ~\textbf{WikiTQ}~              & ~\textbf{TabFact}~             \\ \hline \hline
		Zero-Shot QA   & $17.66$                          & $76.78$                          \\ \hline
		~~~~+ \sys      & $28.22_{\textcolor{cadmiumgreen}{\uparrow 10.56}}$          &              $78.70_{\textcolor{cadmiumgreen}{\uparrow 1.92}}$                   \\
		\hline \hline
		Few-Shot QA     & $56.05$                          & $81.97$                          \\ \hline
		~~~~+ \sys      & $56.33_{\textcolor{cadmiumgreen}{\uparrow 0.28}}$           &             $82.70_{\textcolor{cadmiumgreen}{\uparrow 0.73}}$                \\
		\hline \hline
		% Binder          & $56.98$                          & $79.64$                          \\ \hline
		% ~~~~+ \sys								&			$62.87_{\textcolor{cadmiumgreen}{\uparrow 5.89}}$
		% &  $81.92_{\textcolor{cadmiumgreen}{\uparrow 2.28}}$ \\
		% \hline \hline
		% ReActTable     & $64.25$                          &       $-$                 \\ \hline
		% ~~~~+ \sys      & $\mathbf{65.06_{\textcolor{cadmiumgreen}{\uparrow 0.81}}}$ & $-$ \\
		% \hline \hline
		Text-to-SQL     & $51.66$                          & $68.53$                          \\ \hline
		~~~~+ \sys      & $\mathbf{65.45_{\textcolor{cadmiumgreen}{\uparrow 13.79}}}$ & $\mathbf{86.41_{\textcolor{cadmiumgreen}{\uparrow 17.88}}}$ \\
		\hline
	\end{tabular}
	\label{tbl:different_analyzer}
	\vspace{1mm}
\end{table}

==> tables/existing_work_features.tex <==
%!TEX root = ../main.tex

\begin{table}[t]
  \centering
  \caption{\bf{Comparing \sys with existing TQA methods.}
  }
  %\renewcommand{\arraystretch}{1.12}
  \vspace{-0.5em}
  \scalebox{0.93}{
  \begin{tabular}{|c||c|c|c|c|}
%  |p{3cm}|p{5cm}|
    \hline
    \multirow{2}{*}{\textbf{Method}}   & \textbf{Multiple} & 
    \multicolumn{3}{c|}{\textbf{Supported Data Prep Tasks}} \\
    \cline{3-5}
    & \textbf{Agents} & \textbf{Filter} & \textbf{Derive} & \textbf{Normalize} \\ \hline \hline
    {{Dater~\cite{ye2023large}}}          & \usym{2717}                & \usym{2713}               & \usym{2717}                & \usym{2717}                  \\
    \hline
    {{Binder~\cite{cheng2023binding}}}         & \usym{2717}                & \usym{2717}               & \usym{2713}                & \usym{2717}                  \\
    \hline
    {{CoTable~\cite{wang2024chain}}} & \usym{2717}                & \usym{2713}               & \usym{2713}                & \usym{2717}                  \\
    \hline
    {{ReAcTable~\cite{zhang2024reactable}}}      & \usym{2717}                & \usym{2713}               & \usym{2713}                & \usym{2717}                  \\
    \hline\hline
    {\sys}           & \usym{2713}                & \usym{2713}               & \usym{2713}                & \usym{2713}                  \\
    \hline
  \end{tabular}
  }
  \label{tbl:existing_work_features}
  \vspace{-1em}
\end{table}

==> tables/indepth_analysis_generalization.tex <==
%!TEX root = ../main.tex
\begin{table}[t!]
    \centering
    \caption{\bf{In-depth Analysis of \sys and all baselines on TabBench. AP represents our \sys method.}}
    \vspace{-0.5em}
    % \tabcolsep=0.09cm
    \scalebox{1} {
      \begin{tabular}{|c||c|c|c|}
        \hline
        \multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c|}{\textbf{TabBench}} \\ \cline{2-4}
                                & \textbf{NR}                                                    & \textbf{FC}                                                & \textbf{Overall}      \\
        \hline \hline
        End2End                 & 32.24                                                  & 50.00                                                  & 35.70	\\ \hline
        CoT                     & 23.68                                                  & 44.79                                                  & 27.79	\\ \hline
        NL2Py                   & 40.30                                                  & 44.79                                                  & 41.17 	\\ \hline
        NL2SQL                  & 37.53                                                  & 55.21                                                  & 40.97	\\
        \hline \hline
		ICL-Prep                & 36.02                                                    & 58.33                                                   & 40.36    	\\ \hline
        Dater                   & 26.95                                                    & 51.04                                                   & 30.43 	\\ \hline
        Binder                  & 31.99                                                    & 56.25                                                   & 36.71 	\\ \hline
        ReAcTable               & 41.81                                                    & 57.29                                                   & 44.82 	\\ \hline
        CoTable                 & 27.20                                                    & 59.38                                                   & 33.47 	\\ 
        \hline \hline
        AP {\small + End2End} & $39.80$ 
                                  {\scriptsize \textcolor{cadmiumgreen}{($+7.56$)}}   
                                  & $54.17$ 
                                  {\scriptsize \textcolor{cadmiumgreen}{($+4.17$)}}             
                                  & $42.60$ 
                                  {\scriptsize \textcolor{cadmiumgreen}{($+6.90$)}}             
                                  \\ \hline
        {\small + CoT}       & $37.28$ 
                                  {\scriptsize \textcolor{cadmiumgreen}{($+13.60$)}}    
                                  & $50.00$ 
                                  {\scriptsize \textcolor{cadmiumgreen}{($+5.21$)}}             
                                  & $39.76$ 
                                  {\scriptsize \textcolor{cadmiumgreen}{($+11.97$)}}             
                                  \\ \hline
        {\small + NL2Py}       & $\underline{44.84}$ 
                                  {\scriptsize \textcolor{cadmiumgreen}{($+4.54$)}}    
                                    & $\textbf{60.42}$ 
                                    {\scriptsize \textcolor{cadmiumgreen}{($+15.63$)}}    
                                    & $\underline{47.87}$ 
                                    {\scriptsize \textcolor{cadmiumgreen}{($+6.70$)}}  
                                    \\ \hline
        {\small + NL2SQL }        & $\textbf{46.85}$ 
                                  {\scriptsize \textcolor{cadmiumgreen}{($+9.32$)}}  
                                & $\underline{63.54}$ 
                                {\scriptsize \textcolor{cadmiumgreen}{($+8.33$)}} 
                                & $\textbf{50.10}$ 
                                {\scriptsize \textcolor{cadmiumgreen}{($+9.13$)}}     
                                \\
        \hline
      \end{tabular}
    }
    \vspace{-1em}
    \label{tbl:indepth_analysis_generalization}
  \end{table}
  
  
  
           
             
  
  
  
  

==> tables/indepth_analysis_question_difficulty.tex <==
%!TEX root = ../main.tex
\begin{table}[t!]
  \centering
  \caption{\bf{In-depth Analysis of \sys and all baselines when varying question difficulties on WikiTQ and TabFact.}}
  \vspace{-0.5em}
  % \tabcolsep=0.09cm
  \scalebox{0.88} {
    \begin{tabular}{|c||c|c|c|c|}
      \hline
      \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c|}{\textbf{WikiTQ}} & \multicolumn{2}{c|}{\textbf{TabFact}} \\ \cline{2-5}
                              & \textbf{Simple}                                                         & \textbf{Complex}    & \textbf{Simple}                                                         & \textbf{Complex}     \\
      \hline \hline
      End2End                 & ${57.80}$                                                    & ${55.68}$                                                               & $86.51$  & $77.07$             \\ \hline
      CoT                     & $56.85$                                                                & $55.33$                                                               & ${84.92}$                                                             & ${79.13}$            \\ \hline
      NL2Py                 & ${61.87}$                                                                & ${57.21}$                                                       & $70.83$                                                    & $65.45$  \\ \hline
      NL2SQL                  & $57.02$                                                                & $49.13$                                                               & $70.83$                                                    & $69.59$    \\
      \hline \hline
      ICL-Prep                & ${59.51}$                                                                & ${54.02}$                                                     & $82.64$                                                             & ${78.44}$     \\\hline
	  Dater                   & $51.33$                                                                & $45.77$                                                             & $88.39$ & $77.76$ 														           \\ \hline
      Binder                  & $62.02$                                                                & $52.04$                                                               & $89.29$                                                             & $76.38$                      \\ \hline
      ReAcTable               & ${66.98}$                                                                & ${61.71}$                                                   & ${90.48}$                                                 & ${79.72}$  \\ \hline
      CoTable                 & ${66.88}$                                                                & ${62.53}$                                                     & ${90.58}$                                                    & ${81.89}$     \\ 
      \hline \hline
      AP {\small + End2End}			 & $66.58$ 
								{\scriptsize \textcolor{cadmiumgreen}{($+8.78$)}}   
								& $60.23$ 
								{\scriptsize \textcolor{cadmiumgreen}{($+4.55$)}}             
								& $\underline{87.20}$ 
								{\scriptsize \textcolor{cadmiumgreen}{($+0.69$)}}           
								& $77.07$ 
								{\scriptsize \textcolor{cadmiumgreen}{($+0.00$)}}           
								\\ \hline
      {\small + CoT    }        & $64.12$ 
								{\scriptsize \textcolor{cadmiumgreen}{($+7.27$)}}   
								& $58.57$ 
								{\scriptsize \textcolor{cadmiumgreen}{($+5.24$)}}               
								& $84.52$ 
								{\scriptsize \textcolor{dropred}{($-0.40$)}}           
								& $80.02$ 
								{\scriptsize \textcolor{cadmiumgreen}{($+0.89$)}}             
								\\ \hline
      {\small + NL2Py}       		 & $\underline{68.09}$ 
								{\scriptsize \textcolor{cadmiumgreen}{($+6.22$)}}   
								& $\textbf{63.97}$ 
								{\scriptsize \textcolor{cadmiumgreen}{($+6.76$)}}     
								  & $\textbf{90.77}$ 
								  {\scriptsize \textcolor{cadmiumgreen}{($+19.94$)}} 
								  & $\underline{83.96}$ 
								  {\scriptsize \textcolor{cadmiumgreen}{($+18.51$)}}  
								  \\ \hline
      {\small + NL2SQL }         & $\textbf{69.17}$ 
								{\scriptsize \textcolor{cadmiumgreen}{($+11.97$)}}   
								& $\underline{63.50}$ 
								{\scriptsize \textcolor{cadmiumgreen}{($+14.37$)}}   
							  & $\textbf{90.77}$ 
							  {\scriptsize \textcolor{cadmiumgreen}{($+19.94$)}} 
							  & $\textbf{84.94}$ 
							  {\scriptsize \textcolor{cadmiumgreen}{($+15.35$)}}
							  \\
      \hline
    \end{tabular}
  }
   % \vspace{-1em}  
  \label{tbl:indepth_analysis_question_difficulty}
\end{table}



         
           





==> tables/indepth_analysis_table_size.tex <==
%!TEX root = ../main.tex
\begin{table}[t!]
  \centering
  \caption{\bf{In-depth Analysis of \sys and all baselines when varying different table sizes on WikiTQ. AP represents our \sys method.}}
  \vspace{-0.5em}
  % \tabcolsep=0.09cm
  \scalebox{0.93} {
    \begin{tabular}{|c||c|c|c|}
      \hline
      \multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c|}{\textbf{WikiTQ}} \\ \cline{2-4}
                              & \textbf{Small} {\scriptsize ($<2048$)}                                                          & \textbf{Medium} {\scriptsize ($2048<4096$)}                                                      & \textbf{Large} {\scriptsize ($>4096$)}     \\
      \hline \hline
      End2End                 & ${58.51}$                                                    & $31.00$                                                               & $33.65$             \\ \hline
      CoT                     & $56.56$                                                                & $35.00$                                                               & $30.77$             \\ \hline
      NL2Py                 & ${60.02}$                                                       & ${51.00}$                                                      & ${49.04}$ \\ \hline
      NL2SQL                  & $52.97$                                                                & ${48.00}$                                                   & ${56.73}$    \\
      \hline \hline
      ICL-Prep                & ${56.93}$                                                       & ${48.50}$                                                      & ${56.73}$    \\ \hline
	  Dater                   & $49.03$                                                                & $41.50$                                                               & $33.65$             \\ \hline
      Binder                  & $58.00$                                                                & $51.00$                                                               & $22.12$             \\ \hline
      ReAcTable               & ${64.65}$                                                    & ${62.50}$                                                      & ${47.12}$ \\ \hline
      CoTable                 & ${65.32}$                                                       & ${56.50}$                                                   & ${53.85}$    \\ 
      \hline \hline
      AP {\small + End2End} & $63.86$ 
								{\scriptsize \textcolor{cadmiumgreen}{($+5.35$)}}   
								& $53.00$ 
								{\scriptsize \textcolor{cadmiumgreen}{($+22.00$)}}             
								& $54.81$ 
								{\scriptsize \textcolor{cadmiumgreen}{($+21.16$)}}             
								\\ \hline
      {\small + CoT}       & $62.22$ 
								{\scriptsize \textcolor{cadmiumgreen}{($+5.66$)}}    
								& $45.00$ 
								{\scriptsize \textcolor{cadmiumgreen}{($+10.00$)}}             
								& $49.04$ 
								{\scriptsize \textcolor{cadmiumgreen}{($+18.27$)}}             
								\\ \hline
      {\small + NL2Py}       & $\underline{66.01}$ 
								{\scriptsize \textcolor{cadmiumgreen}{($+5.99$)}}    
								  & $\textbf{67.50}$ 
								  {\scriptsize \textcolor{cadmiumgreen}{($+16.50$)}}    
								  & $\underline{56.73}$ 
								  {\scriptsize \textcolor{cadmiumgreen}{($+7.69$)}}  
								  \\ \hline
      {\small + NL2SQL }        & $\textbf{66.29}$ 
								{\scriptsize \textcolor{cadmiumgreen}{($+13.32$)}}  
							  & $\underline{64.00}$ 
							  {\scriptsize \textcolor{cadmiumgreen}{($+16.00$)}} 
							  & $\textbf{62.50}$ 
							  {\scriptsize \textcolor{cadmiumgreen}{($+5.77$)}}     
							  \\
      \hline
    \end{tabular}
  }
  \vspace{-1em}
  \label{tbl:indepth_analysis_table_size}
\end{table}



         
           





==> tables/llm_code_for_op_analysis.tex <==
\begin{table}[t]
    \centering
    \caption{\bf{Analyzing LLM generated code for logical operator.}}
    \label{tbl:llm_code_for_op_analysis}
    \vspace{-0.5em}
    \resizebox{0.65\linewidth}{!}{
    \begin{tabular}{|c||c|}
        \hline
        \textbf{Method} & ~\textbf{WikiTQ}~  \\ \hline \hline
        $\mathtt{CustomCode}$ ratio & ${1.08\%}$  \\ \hline
        $\mathtt{CustomCode}$ accuracy & ${55.32\%}$ \\ \hline \hline
        
        \sys w. $\mathtt{CustomCode}$ & $\textbf{66.09}$\\ \hline
        \sys w.o. $\mathtt{CustomCode}$ & ${65.63}$  \\ 
        \hline
    \end{tabular}
    }
\end{table}


% 47 个case调用$\mathtt{CustomCode}$


==> tables/overall_comparisons.tex <==
%!TEX root = ../main.tex
\begin{table}[t!]
    \centering
    \caption{\bf{Comparison of \sys with data prep methods for TQA (the best results are bolded, and the second-best results are underlined).} 
    }
   \vspace{-0.5em}
   %\vspace{-1em}
    \renewcommand{\arraystretch}{1.2}
    % \tabcolsep=0.2cm
    \scalebox{1}{
    \begin{tabular}{|c||c|c|c|c|}
        \hline
         \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c|}{\textbf{DeepSeek}} & \multicolumn{2}{c|}{\textbf{GPT3.5}} \\ \cline{2-5}
		& \textbf{WikiTQ}  & \textbf{TabFact} & \textbf{WikiTQ}  & \textbf{TabFact}  \\
        \hline \hline
  %       Zero-Shot QA                      & $17.66$                                      & $76.78$                                      & $51.84$                                      & $70.45$  \\ \cline{1-5} % [1pt]
		% Few-Shot QA                      & $56.05$                                      & $\underline{81.97}$


           
  %                                     & $52.56$                                      & $71.54$  \\ \cline{1-5} % [1pt]
  %                                         % & Chain-of-Thought                      &  50.36                                     &                                       & $53.48$                                      & $65.37$  \\  % [1pt]
  %       \hline \hline      
		% Text-to-SQL                      & $51.66$                                      & $68.53$                                      & $52.90$                                      & $64.71$  \\ \cline{1-5} % [1pt]
		Binder                      & $56.98$                                      & $79.64$                                      & $\underline{56.74}$                                      & $\underline{79.17}$
           \\ \cline{1-5} % [1pt]
                                          % & Dater                      &                                       &                                       & 52.81                                      & 78.01 % \\ \cline{1-5} % [1pt]
        ReAcTable                      &     $\underline{64.25}$                                   &   $-$                                    & $51.80$                                      & $72.80$     \\  
        \hline \hline
		\sys         & $\mathbf{65.45}$                                       & $\mathbf{86.41}$ (87.01)                                      & $\mathbf{63.86}$                                      &   $\mathbf{84.29}$     \\ % rerun the experiments and update performance on GPT3.5
	  \hline
    \end{tabular}}
    \label{tbl:overall_comparisons}
\end{table}

==> tables/planner_variants.tex <==
\begin{table}[t!]
	\centering
	\caption{\bf{Comparison of different Methods for \textsc{Planner}.}}
        % \tabcolsep=0.45cm
	%\renewcommand{\arraystretch}{1.12}
   \vspace{-0.5em}
	\begin{tabular}{|c||c|c|c|}
		\hline
		\textbf{Method} & ~\textbf{WikiTQ}~              & ~\textbf{TabFact}~    & ~\textbf{TabBench}~             \\ \hline \hline
		Direct Prompting   & $58.17$                          & $83.35$        & $44.83$                          \\ \hline
		Chain-of-Clauses      & $\textbf{66.09}$          &              $\textbf{87.85}$      &              $\textbf{50.10}$                   \\ 
		\hline
	\end{tabular}
	\label{tbl:planner_variants}
	\vspace{-1mm}
\end{table}	


==> tables/programmer_varients.tex <==
\begin{table}[t!]
	\centering
	\caption{\bf{Comparison of different Methods for \textsc{Programmer}, where Acc. represents TQA accuracy and Err. represents the ratio of code errors. The highest Acc. and lowest Err. are bolded.}}
        % \tabcolsep=0.45cm
	%\renewcommand{\arraystretch}{1.12}
   \vspace{-0.5em}
	\begin{tabular}{|c|c||c|c|c|}
		\hline
		\textbf{Method} & \textbf{Metric} & ~\textbf{WikiTQ}~              & ~\textbf{TabFact}~    & ~\textbf{TabBench}~             \\ \hline \hline
		\multirow{2}{*}{Code-generation} & Acc $\uparrow$     & $62.82$           &             $81.97$         &              $47.26$                     \\ \cline{2-5}
													& Err $\downarrow$ & $4.51\%$          & $4.50\%$  & $4.73\%$                     \\ \hline
		\multirow{2}{*}{Tool-augmented}  & Acc $\uparrow$     & $\textbf{66.09}$          &              $\textbf{87.85}$       &              $\textbf{50.10}$   \\  \cline{2-5}
													& Err $\downarrow$ & $\textbf{1.50\%}$          &              $\textbf{0.05\%}$   &              $\textbf{1.01\%}$    \\
		  
		\hline
	\end{tabular}
	\label{tbl:programmer_varients}
	\vspace{-1mm}
\end{table}	

==> tables/tabfact_answer_format_error.tex <==
\begin{table*}[t]
    \centering
    \caption{\bf{Answer Format Error Case in TabFact Dataset.}}
    \label{tbl:tabfact_answer_format_error}
    \vspace{-0.5em}
    \resizebox{0.75\linewidth}{!}{
    \begin{tabular}{|c|l|}
        \hline
\textbf{Category}   & TabFact-Answer Format Error                                                               \\ \hline\hline
\textbf{Table}      & \makecell[l]{row\_id | aircraft | origin | type | versions | in service\\
---|---|---|---|---|---\\
1 | cessna a - 37 dragonfly | united states | attack / fighter | a - 37b | 12 (16 delivered)\\
2 | fma ia 58 pucarã¡ | argentina | attack | a - 58 | 5 (6 delivered)\\
3 | lockheed c - 130 hercules | united states | transport / utility | c - 130b | 2\\
4 | embraer emb 110 bandeirante | brazil | transport / utility | c - 95 | 3\\
5 | beechcraft twin bonanza | united states | transport / utility | d50 | 1\\
6 | casa c - 212 aviocar | spain | transport | c - 212 - 200 | 2\\
7 | embraer emb 120 brasilia | brazil | transport | emb 120 | 1\\
8 | cessna 206 stationair | united states | utility / liaison | u206h | 10\\
9 | beechcraft b58 baron | united states | trainer / liaison | b - 58 | 2\\
10 | british aerospace 125 | united kingdom | vip transport | 700a 600a | 2\\
11 | aermacchi sf260 | italy | trainer | t - 260 eu | 12\\
12 | pilatus pc - 7 turbo trainer | switzerland | trainer | - 92 | 5 (6 delivered)\\
13 | cessna t - 41 mescalero | united states | trainer | t - 41d | 7\\
14 | aerospatiale as 365 dauphin | france | liaison / transport | as 365 | 1\\
15 | bell 212 twin huey | united states | transport / utility | bell 212 | 4\\
16 | bell uh - 1 iroquois | united states | transport / utility | uh - 1h | 13}                                                                  \\\hline
\textbf{Statement}   & the aircraft bell 212 twin huey was a trainer type                                                      \\\hline
\textbf{Label}      & false                                                                        \\ \hline\hline
\textbf{SQL}        & \makecell[l]{SELECT `type` FROM w WHERE `aircraft` = "bell 212 twin huey" ;}                                        \\\hline
\textbf{Prediction} & transport / utility                                                                     \\ \hline\hline
\textbf{Reason}     & \makecell[l]{It requires the answer to be in the form of a boolean value,\\but the prediction is a string.}
       \\ \hline
    \end{tabular}
    }
\end{table*}

==> tables/tabfact_reasoning_error.tex <==
\begin{table*}[t]
    \centering
    \caption{\bf{Reasoning Error Case in TabFact Dataset.}}
    \label{tbl:tabfact_reasoning_error}
    \vspace{-0.5em}
    \resizebox{0.99\linewidth}{!}{
    \begin{tabular}{|c|l|}
        \hline
\textbf{Category}   & TabFact-Reasoning Error                                                               \\ \hline\hline
\textbf{Table}      & \makecell[l]{row\_id | party | administrative panel | agricultural panel | cultural and educational panel | industrial and commercial panel |\\labour panel | national university of ireland | university of dublin | nominated by the taoiseach | total\\
---|---|---|---|---|---|---|---|---|---|---\\
1 | fianna fáil | 4 | 4 | 2 | 3 | 0 | 1 | 0 | 7 | 21\\
2 | fine gael | 1 | 3 | 2 | 2 | 0 | 1 | 0 | 0 | 9\\
3 | labour party | 0 | 0 | 0 | 1 | 5 | 0 | 0 | 2 | 8\\
4 | clann na talmhan | 0 | 2 | 0 | 0 | 1 | 0 | 0 | 0 | 3\\
5 | independent | 0 | 1 | 0 | 1 | 0 | 1 | 3 | 3 | 9\\
6 | total | 7 | 11 | 5 | 9 | 11 | 3 | 3 | 11 | 60}                                                                  \\\hline
\textbf{Statement}   & industrial and commercial panel has four more members than cultural and educational panel                                                      \\\hline
\textbf{Label}      & true                                                                        \\ \hline\hline
\textbf{SQL}        & \makecell[l]{SELECT ( SELECT COUNT ( * ) FROM w WHERE `industrial and commercial panel` IS NOT null ) - \\( SELECT COUNT ( * ) FROM w WHERE `cultural and educational panel` IS NOT null ) = 4}                                        \\\hline
\textbf{Prediction} & false                                                                     \\ \hline\hline
% SQL 查询的逻辑是计算 industrial and commercial panel 和 cultural and educational panel 的成员数量差异，但查询中使用了 COUNT(*) 来统计非空行数，而不是直接比较两列的总和（即 SUM）。这导致未能正确找到相关值，从而得出错误结果。正确的做法应该是使用 SUM 函数来计算两列的总和并比较差异。
\textbf{Reason}     & \makecell[l]{The SQL query logic is to calculate the difference in the number of members between the `industrial and commercial\\panel` and `cultural and educational panel`. However, it uses COUNT(*) to count non-null rows instead of directly\\comparing the sums of the two columns (i.e., SUM). This leads to an incorrect result. The correct approach should\\be to use the SUM function to calculate the totals of both columns and compare the difference.}
       \\ \hline
    \end{tabular}
    }
\end{table*}

==> tables/tabfact_unclear_question.tex <==
\begin{table*}[t]
    \centering
    \caption{\bf{Unclear Question Case in TabFact Dataset.}}
    \label{tbl:tabfact_unclear_question}
    \vspace{-0.5em}
    \resizebox{0.8\linewidth}{!}{
    \begin{tabular}{|c|l|}
        \hline
\textbf{Category}   & TabFact-Unclear Question                                                               \\ \hline\hline
\textbf{Table}      & \makecell[l]{row\_id | district | incumbent | party | first elected | status | opponent\\
---|---|---|---|---|---|---\\
1 | pennsylvania4 | ron klink | democratic | 1992 | re - elected | ron klink (d) 64.2\% ed peglow (r) 35.8\%\\
2 | pennsylvania5 | william f clinger , jr | republican | 1978 | re - elected | william f clinger , jr (r) unopposed\\
3 | pennsylvania7 | curt weldon | republican | 1986 | re - elected | curt weldon (r) 69.7\% sara r nichols (d) 30.3\%\\
4 | pennsylvania9 | bud shuster | republican | 1972 | re - elected | bud shuster (r) unopposed\\
5 | pennsylvania12 | john murtha | democratic | 1974 | re - elected | john murtha (d) 68.9\% bill choby (r) 31.1\%\\
6 | pennsylvania17 | george gekas | republican | 1982 | re - elected | george gekas (r) unopposed\\
7 | pennsylvania18 | rick santorum | republican | 1990 | retired to run for us senate democratic gain | michael...\\
8 | pennsylvania19 | william f goodling | republican | 1974 | re - elected | william f goodling (r) unopposed}                                                                  \\\hline
\textbf{Statement}   & william f goodling was one of six republican incumbents to be re - elected                                                      \\\hline
\textbf{Label}      & true                                                                        \\ \hline\hline
\textbf{SQL}        & \makecell[l]{SELECT \\( SELECT COUNT ( * ) FROM w WHERE `party` = "republican" and `status` = "re - elected" ) = 6 and \\( SELECT COUNT ( * ) FROM w WHERE `incumbent` = "william f goodling" and `status` = "re - elected" ) = 1 ;}                                        \\\hline
\textbf{Prediction} & false                                                                     \\ \hline\hline
\textbf{Reason}     & \makecell[l]{It is unclear whether the statement claims that there are six republican incumbents who were re-elected or \\that william f goodling was to be re-elected and one of six republican incumbents.}
       \\ \hline
    \end{tabular}
    }
\end{table*}

==> tables/wikitq_answer_format_error.tex <==
\begin{table*}[t]
    \centering
    \caption{\bf{Answer Format Error Case in WikiTQ Dataset.}}
    \label{tbl:wikitq_answer_format_error}
    \vspace{-0.5em} % 可选，视情况调整
    \resizebox{0.65\linewidth}{!}{
    \begin{tabular}{|c|l|}
        \hline
\textbf{Category}   & WikiTQ-Answer Format Error                                                               \\ \hline\hline
\textbf{Table}      & \makecell[l]{row\_id | Client | Years of Operation | Area of Operation | Country | Services\\ 
---|---|---|---|---|---\\ 
1 | Agoco | 1991-current | Sarir field | Libya | Drilling, workover\\ 
2 | Lasmo | 1993-94 | Wadi Borjuj | Libya | Drilling, workover\\ 
3 | Waha | 1994 | El Zahra | Libya | Drilling, workover\\ 
4 | IPC-Dublin | 1997-97 | Kilwa | Tanzania | Drilling\\ 
5 | OMV | 1997 | Field 103 | Libya | Drilling, workover\\ 
6 | Fina | 1997 | El Hamada | Libya | Drilling, workover\\ 
7 | Marathon | 1998 | Manzala field | Egypt | Drilling\\ 
8 | Khalda/Repsol | 1998-99 | West Desert | Egypt | Drilling\\ 
9 | Total | 1999-current | El Mabrouk | Libya | Drilling\\ 
10 | Agiba-Agip | 1999 | West Desert | Egypt | Drilling\\ 
11 | IPLL | 1999-current | El Naka field | Libya | Drilling\\ 
12 | SOC | 2000-current | SOC fields | Libya | Drilling\\ 
13 | Veba | 2000 | Different fields | Libya | Drilling, workover\\ 
14 | Perenco Oil Co. | 2000-01 | EchiraX Concession | Gabon | Drilling\\ 
15 | Zueitina | 2001-current | Field 103 | Libya | Drilling, workover}                                                                  \\\hline
\textbf{Question}   & which country has the greatest number of challenger operations?                                                      \\\hline
\textbf{Label}      & Libya                                                                        \\ \hline\hline
\textbf{SQL}        & \makecell[l]{SELECT `Country` , COUNT ( * ) AS `operation\_count` FROM w\\GROUP by `Country` ORDER by `operation\_count` desc LIMIT 1 ;}                                        \\\hline
\textbf{Prediction} & Libya|10                                                                     \\ \hline\hline
\textbf{Reason}     & Extract extra information `operation\_count` in the SQL.
       \\ \hline
    \end{tabular}
    }
\end{table*}

==> tables/wikitq_evaluation_error.tex <==
\begin{table*}[t]
    \centering
    \caption{\bf{Evaluation Error Case in WikiTQ Dataset.}}
    \label{tbl:wikitq_evaluation_error}
    \vspace{-0.5em} % 可选，视情况调整
    \resizebox{0.8\linewidth}{!}{
    \begin{tabular}{|c|l|}
        \hline
\textbf{Category}   & WikiTQ-Evaluation Error                                                               \\ \hline\hline
\textbf{Table}      & \makecell[l]{row\_id | Week | Date | TV Time | Opponent | Result | Attendance\\
---|---|---|---|---|---|---\\
1 | 1 | September 6, 1998 | FOX 1:05 pm MT | at Dallas Cowboys | L 38–10 | 63,602\\
2 | 2 | September 13, 1998 | FOX 1:15 pm MT | at Seattle Seahawks | L 33–14 | 57,678\\
3 | 3 | September 20, 1998 | ESPN 5:15 pm MT | Philadelphia Eagles | W 17–3 | 39,782\\
4 | 4 | September 27, 1998 | FOX 10:00 am MT | at St. Louis Rams | W 20–17 | 55,832\\
5 | 5 | October 4, 1998 | CBS 1:05 pm MT | Oakland Raiders | L 23–20 | 53,240\\
6 | 6 | October 11, 1998 | FOX 1:05 pm MT | Chicago Bears | W 20–7 | 50,495\\
7 | 7 | October 18, 1998 | FOX 10:00 am MT | at New York Giants | L 34–7 | 70,456\\
8 | 8 | Bye | Bye | Bye | Bye | nan\\
9 | 9 | November 1, 1998 | FOX 11:00 am MT | at Detroit Lions | W 17–15 | 66,087\\
10 | 10 | November 8, 1998 | FOX 2:15 pm MT | Washington Redskins | W 29–27 | 45,950\\
11 | 11 | November 15, 1998 | FOX 2:15 pm MT | Dallas Cowboys | L 35–28 | 71,670\\
12 | 12 | November 22, 1998 | FOX 11:00 am MT | at Washington Redskins | W 45–42 | 63,435\\
13 | 13 | November 29, 1998 | FOX 11:00 am MT | at Kansas City Chiefs | L 34–24 | 69,613\\
14 | 14 | December 6, 1998 | FOX 2:15 pm MT | New York Giants | L 23–19 | 46,128\\
15 | 15 | December 13, 1998 | FOX 11:00 am MT | at Philadelphia Eagles | W 20–17 | 62,176\\
16 | 16 | December 20, 1998 | FOX 2:05 pm MT | New Orleans Saints | W 19–17 | 51,617\\
17 | 17 | December 27, 1998 | CBS 2:05 pm MT | San Diego Chargers | W 16–13 | 71,670}                                                                  \\\hline
\textbf{Question}   & who was the first game against?                                                       \\\hline
\textbf{Label}      & Dallas Cowboys                                                                        \\ \hline\hline
\textbf{SQL}        & SELECT 'Opponent' FROM w WHERE 'week' = "1"                                           \\\hline
\textbf{Prediction} & at Dallas Cowboys                                                                     \\ \hline\hline
\textbf{Reason}     & Fail to match "Dallas Cowboys" and "at Dalls Cowboys" which are semantically matched.
       \\ \hline
    \end{tabular}
    }
\end{table*}

==> tables/wikitq_labeling_error.tex <==
\begin{table*}[t]
    \centering
    \caption{\bf{Labeling Error Case in WikiTQ Dataset.}}
    \label{tbl:wikitq_labeling_error}
    \vspace{-0.5em} % 可选，视情况调整
    \resizebox{0.8\linewidth}{!}{
    \begin{tabular}{|c|l|}
        \hline
\textbf{Category}   & WikiTQ-Labeling Error                                                               \\ \hline\hline
\textbf{Table}      & \makecell[l]{row\_id | May 20-21 118 | March 9 120 | December 25-26 122 | October 13-14 124 | August 1-2 126\\
---|---|---|---|---|---\\
1 | May 21, 1993 | March 9, 1997 | December 25, 2000 | October 14, 2004 | August 1, 2008\\
2 | 128 | 130 | 132 | 134 | 136\\
3 | May 20, 2012 | March 9, 2016 | December 26, 2019 | October 14, 2023 | August 2, 2027\\
4 | 138 | 140 | 142 | 144 | 146\\
5 | May 21, 2031 | March 9, 2035 | December 26, 2038 | October 14, 2042 | August 2, 2046\\
6 | 148 | 150 | 152 | 154 | 156\\
7 | May 20, 2050 | March 9, 2054 | December 26, 2057 | October 13, 2061 | August 2, 2065}                                                                  \\\hline
\textbf{Question}   & what is the date of the last solar eclipse listed?                                                      \\\hline
\textbf{Label}      & 20-May-69                                                                        \\ \hline\hline
\textbf{SQL}        & \makecell[l]{SELECT `August 1-2 126` FROM w WHERE `row\_id` = ( SELECT MAX ( `row\_id` ) FROM w )}                                        \\\hline
\textbf{Prediction} & August 2, 2065                                                                     \\ \hline\hline
\textbf{Reason}     & \makecell[l]{The label is incorrect because both the value and the format are wrong. \\The correct label should be ``August 2, 2065''.}
       \\ \hline
    \end{tabular}
    }
\end{table*}

==> tables/wikitq_unclear_question.tex <==
\begin{table*}[t]
    \centering
    \caption{\bf{Unclear Question Case in WikiTQ Dataset.}}
    \label{tbl:wikitq_unclear_question}
    \vspace{-0.5em} % 可选，视情况调整
    \resizebox{0.99\linewidth}{!}{
    \begin{tabular}{|c|l|}
        \hline
\textbf{Category}   & WikiTQ-Unclear Question Error                                                               \\ \hline\hline
\textbf{Table}      & \makecell[l]{row\_id | Date | Competition | Location | Country | Event | Placing | Rider | Nationality\\
---|---|---|---|---|---|---|---|---\\
1 | 31 October 2008 | 2008-09 World Cup | Manchester | United Kingdom | Sprint | 1 | Victoria Pendleton | GBR\\
2 | 31 October 2008 | 2008-09 World Cup | Manchester | United Kingdom | Keirin | 2 | Jason Kenny | GBR\\
3 | 1 November 2008 | 2008-09 World Cup | Manchester | United Kingdom | Sprint | 1 | Jason Kenny | GBR\\
4 | 1 November 2008 | 2008-09 World Cup | Manchester | United Kingdom | 500 m time trial | 1 | Victoria Pendleton | GBR\\
5 | 2 November 2008 | 2008-09 World Cup | Manchester | United Kingdom | Team sprint | 1 | Ross Edgar | GBR\\
6 | 2 November 2008 | 2008-09 World Cup | Manchester | United Kingdom | Team sprint | 1 | Jason Kenny | GBR\\
7 | 2 November 2008 | 2008-09 World Cup | Manchester | United Kingdom | Team sprint | 1 | Jamie Staff | GBR\\
8 | 2 November 2008 | 2008-09 World Cup | Manchester | United Kingdom | Keirin | 1 | Victoria Pendleton | GBR\\
9 | 2 November 2008 | 5th International Keirin Event | Manchester | United Kingdom | International keirin | 2 | Ross Edgar | GBR\\
10 | 13 February 2009 | 2008-09 World Cup | Copenhagen | Denmark | Team sprint | 1 | Chris Hoy | GBR\\
11 | 13 February 2009 | 2008-09 World Cup | Copenhagen | Denmark | Team sprint | 1 | Jason Kenny | GBR\\
12 | 13 February 2009 | 2008-09 World Cup | Copenhagen | Denmark | Team sprint | 1 | Jamie Staff | GBR\\
13 | 13 February 2009 | 2008-09 World Cup | Copenhagen | Denmark | Sprint | 1 | Victoria Pendleton | GBR\\
14 | 30 October 2009 | 2009-10 World Cup | Manchester | United Kingdom | Keirin | 1 | Chris Hoy | GBR\\
15 | 30 October 2009 | 2009-10 World Cup | Manchester | United Kingdom | Sprint | 1 | Victoria Pendleton | GBR\\
16 | 30 October 2009 | 2009-10 World Cup | Manchester | United Kingdom | Sprint | 1 | Chris Hoy | GBR\\
17 | 30 October 2009 | 2009-10 World Cup | Manchester | United Kingdom | 500 m time trial | 2 | Victoria Pendleton | GBR\\
18 | 1 November 2009 | 2009-10 World Cup | Manchester | United Kingdom | Team sprint | 1 | Ross Edgar | GBR\\
19 | 1 November 2009 | 2009-10 World Cup | Manchester | United Kingdom | Team sprint | 1 | Chris Hoy | GBR\\
20 | 1 November 2009 | 2009-10 World Cup | Manchester | United Kingdom | Team sprint | 1 | Jamie Staff | GBR}                                                                  \\\hline
\textbf{Question}   & what is the total number of competition?                                                      \\\hline
\textbf{Label}      & 20                                                                        \\ \hline\hline
\textbf{SQL}        & \makecell[l]{SELECT COUNT ( distinct `Competition` ) FROM w}                                        \\\hline
\textbf{Prediction} & 3                                                                     \\ \hline\hline
\textbf{Reason}     & It is unclear whether the question is asking for the number of distinct competitions or the total number of rows in the table.
       \\ \hline
    \end{tabular}
    }
\end{table*}

==> tables/wikitq_value_retrieval_error.tex <==
\begin{table*}[t]
    \centering
    \caption{\bf{Value Retrieval Error Case in WikiTQ Dataset.}}
    \label{tbl:wikitq_value_retrieval_error}
    \vspace{-0.5em} % 可选，视情况调整
    \resizebox{0.65\linewidth}{!}{
    \begin{tabular}{|c|l|}
        \hline
\textbf{Category}   & WikiTQ-Value Retrieval Error                                                               \\ \hline\hline
\textbf{Table}      & \makecell[l]{row\_id | Team | No | Driver | Class | Rounds\\
---|---|---|---|---|---\\
1 | Josef Kaufmann Racing | 4 | Robin Frijns | nan | All\\
2 | Josef Kaufmann Racing | 5 | Hannes van Asseldonk | R | All\\
3 | Josef Kaufmann Racing | 6 | Petri Suvanto | R | All\\
4 | Mücke Motorsport | 7 | Maciej Bernacik | R | All\\
5 | Mücke Motorsport | 8 | Timmy Hansen | nan | All\\
6 | EuroInternational | 11 | Daniil Kvyat | R | All\\
7 | EuroInternational | 12 | Carlos Sainz, Jr. | R | All\\
8 | EuroInternational | 14 | Michael Lewis | nan | All\\
9 | DAMS | 15 | Javier Tarancón | nan | All\\
10 | DAMS | 16 | Dustin Sofyan | nan | 5\\
11 | DAMS | 16 | Luciano Bacheta | nan | 7-8\\
12 | DAMS | 17 | Fahmi Ilyas | nan | 1-6\\
13 | DAMS | 17 | Dustin Sofyan | nan | 8\\
14 | Eifelland Racing | 18 | Facundo Regalia | nan | All\\
15 | Eifelland Racing | 19 | Côme Ledogar | nan | All\\
16 | Eifelland Racing | 20 | Marc Coleselli | R | All\\
17 | Fortec Motorsport | 24 | Jack Harvey | nan | All\\
18 | Fortec Motorsport | 25 | George Katsinis | nan | All\\
19 | Fortec Motorsport | 26 | Christof von Grünigen | nan | All}                                                                  \\\hline
\textbf{Question}   & what are the total number of times all appears under the rounds column?                                                      \\\hline
\textbf{Label}      & 15                                                                        \\ \hline\hline
\textbf{SQL}        & \makecell[l]{SELECT COUNT ( * ) FROM w WHERE `Rounds` = "all"}                                        \\\hline
\textbf{Prediction} & 0                                                                     \\ \hline\hline
\textbf{Reason}     & \makecell[l]{The SQL query is correct, but the prediction is incorrect because the model\\fails to count the number of rows with "All" in the `Rounds` column.}
       \\ \hline
    \end{tabular}
    }
\end{table*}
